Progressive Open Space Expansion for Open-Set Model Attribution

Despite the remarkable progress in generative technology, the Janus-faced issues of intellectual property protection and malicious content supervision have arisen. Efforts have been paid to manage synthetic images by attributing them to a set of potential source models. However, the closed-set classification setting limits the application in real-world scenarios for handling contents generated by arbitrary models. In this study, we focus on a challenging task, namely Open-Set Model Attribution (OSMA), to simultaneously attribute images to known models and identify those from unknown ones. Compared to existing open-set recognition (OSR) tasks focusing on semantic novelty, OSMA is more challenging as the distinction between images from known and unknown models may only lie in visually imperceptible traces. To this end, we propose a Progressive Open Space Expansion (POSE) solution, which simulates open-set samples that maintain the same semantics as closed-set samples but embedded with different imperceptible traces. Guided by a diversity constraint, the open space is simulated progressively by a set of lightweight augmentation models. We consider three real-world scenarios and construct an OSMA benchmark dataset, including unknown models trained with different random seeds, architectures, and datasets from known ones. Extensive experiments on the dataset demonstrate POSE is superior to both existing model attribution methods and off-the-shelf OSR methods.

==> Figures/ablation_K.tex <==
\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=0.8\linewidth]{Images/K_along_epoch3.pdf}
% \vspace{-4pt}
\caption{The influence of the number of augmentation models to open-set recognition performance.}
\vspace{-5mm}
\label{fig:ablation_K}
\end{figure}

==> Figures/ablation_arch.tex <==


% \newcommand\pecomparisonfigurewidth{}

% \begin{figure}%[b]
% \setlength{\abovecaptionskip}{2mm}
% \centering
% \includegraphics[width=0.32\linewidth]{Images/arch_ablation/kernel_size.pdf}
% \includegraphics[width=0.32\linewidth]{Images/arch_ablation/layer_num.pdf}
% \includegraphics[width=0.32\linewidth]{Images/arch_ablation/up.png}
% \vspace{-4pt}
% \caption{The influence of kernel size, layer num and upsample layer.}
% \vspace{-5mm}
% \label{fig:ablation_arch}
% \end{figure}


\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering
% \includegraphics[width=0.26\linewidth]{Images/arch_ablation/up_bar_d0.95.png}
% \includegraphics[width=0.35\linewidth]{Images/arch_ablation/layer_num_bar_d0.95.png}
% \includegraphics[width=0.35\linewidth]{Images/arch_ablation/kernel_size_bar_d0.95.png}
\includegraphics[width=0.26\linewidth]{Images/arch_ablation/up_bar_d0.95_POSE.png}
\includegraphics[width=0.35\linewidth]{Images/arch_ablation/layer_num_bar_d0.95_new.png}
\includegraphics[width=0.35\linewidth]{Images/arch_ablation/kernel_size_bar_d0.95_POSE.png}
\begin{minipage}[t]{0.28\linewidth}
    \centering
    \figtext{(a) Upsampling}
\end{minipage}
\begin{minipage}[t]{0.35\linewidth}
    \centering
    \figtext{(b) Layer number}
\end{minipage}
\begin{minipage}[t]{0.35\linewidth}
    \centering
    \figtext{(c) Kernel size}
\end{minipage}
\caption{Ablation study on the architecture of augmentation models. We consider whether to include a upsample layer, layer number and kernel size of convolution layers.}
\label{fig:ablation_arch}
\vspace{-7mm}
\end{figure}

==> Figures/case.tex <==

\newcommand\casewidth{0.24}
\begin{figure}[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\casewidth\linewidth]{Images/case2/tsne-epoch29-case_base_celeba_ProGAN_seed0_celeba_MMDGAN.pdf}
\includegraphics[width=\casewidth\linewidth]{Images/case2/tsne-epoch29-case_base_stylegan3_cat_sngan_cat.pdf}
\includegraphics[width=\casewidth\linewidth]{Images/case2/tsne-epoch24-case_celeba_ProGAN_seed0_celeba_MMDGAN2.pdf}
\includegraphics[width=\casewidth\linewidth]{Images/case2/tsne-epoch24-case_stylegan3_cat_sngan_cat2.pdf}
% \vspace{-4pt}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{(a) Base}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{(b) POSE}
\end{minipage}
\caption{Feature space visualization for Base method and POSE.}
\label{fig:case}
\vspace{-5mm}
\end{figure}


% \begin{figure}[!t]
% \setlength{\abovecaptionskip}{2mm}
% \centering
% \includegraphics[width=\linewidth]{Images/case.pdf} 
% \caption{Open space expansion helps to reject unknown classes.}   
% \label{fig:intro}
% \vspace{-5mm}
% \end{figure}


% \begin{figure}%[b]
% \setlength{\abovecaptionskip}{2mm}
% \centering
% \includegraphics[width=0.8\linewidth]{Images/case.pdf}

% \begin{minipage}[t]{0.45\linewidth}
%     \centering
%     \figtext{(a) Base}
% \end{minipage}
% \begin{minipage}{0.1\linewidth}
%     \centering
%     \figtext{\quad}
% \end{minipage}
% \begin{minipage}[t]{0.4\linewidth}
%     \centering
%     \figtext{(b) POSE}
% \end{minipage}
% \caption{Confidence histograms for base model and POSE.}
% \label{fig:hist_compare}
% \vspace{-5mm}
% \end{figure}

==> Figures/dataset_explain1.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1.0\linewidth]{Images/dataset_explain1.png} 
\end{center}
  \caption{The relationship between seen fake and unseen fake.}   
\label{fig:dataset_explain1}
\end{figure}


==> Figures/dataset_explain2.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=1.0\linewidth]{Images/dataset_explain2.png} 
\end{center}
  \caption{Data Split. The benchmark contains training and testing set. The testing set is further divided into closed-set and open-set testing set.}   
\label{fig:dataset_explain2}
\end{figure}


==> Figures/diffusion_hist.tex <==
\begin{figure}[htbp]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=0.8\linewidth]{Images/diffusion/diffusion_hist-d0.95.pdf}
% \vspace{-4pt}
\caption{Confidence histograms on unseen stable diffusion data and closed-set data.}
\vspace{-5mm}
\label{fig:diffusion_hist}
\end{figure}

==> Figures/diffusion_samples.tex <==

\newcommand\diffusionsamplewidth{0.195}
\begin{figure*}[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/diffusion/a_blue_train_in_the_middle_of_a_forest.png}
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/diffusion/A_chain_link_fence_contains_a_building_and_rubbish_.png}
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/diffusion/A_clock_sits_high_on_a_wall_while_below_it_on_the_wall_features_mosaic_tiles.png}
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/diffusion/A_group_of_people_in_a_field_smile_holding_frisbees.png}
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/diffusion/A_soccer_player_trying_to_score_a_goal.png}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(a) A blue train in the middle of a forest.}
\end{minipage}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(b) A chain link fence contains a building and rubbish.}
\end{minipage}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(c) A clock sits high on a wall while below it on the wall features mosaic tiles.}
\end{minipage}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(d) A group of people in a field smile holding frisbees.}
\end{minipage}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(e) A soccer player trying to score a goal.}
\end{minipage}
\caption{Randomly selected samples generated by the stable diffusion model.}
\label{fig:diffusion_samples}
% \vspace{-5mm}
\end{figure*}

==> Figures/feasibility.tex <==
\newcommand\pecomparisonfigurewidth{0.47}

\begin{figure}[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\begin{minipage}{0.04\linewidth}
    \centering
    \rotatebox{90}{}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{\scriptsize StyleGAN3\_FFHQ}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{\scriptsize StyleGAN\_Bus}
\end{minipage}
\begin{minipage}[t]{0.04\linewidth}
    \centering
    \rotatebox{90}{\scriptsize \hspace{0.5cm}(a)}
\end{minipage}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/feasibility/arch/input0.png}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/feasibility/data/input0.png}

\vspace{-4pt}
\begin{minipage}{0.04\linewidth}
    \centering
    \rotatebox{90}{}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{\scriptsize StyleGAN2\_FFHQ}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{\scriptsize StyleGAN\_Cat}
\end{minipage}
\begin{minipage}[t]{0.04\linewidth}
    \centering
    \rotatebox{90}{\scriptsize \hspace{0.5cm}(b)}
\end{minipage}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/feasibility/arch/input1.png}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/feasibility/data/input1.png}

\vspace{-4pt}
\begin{minipage}{0.04\linewidth}
    \centering
    \rotatebox{90}{}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{\scriptsize A(StyleGAN3\_FFHQ)}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{\scriptsize A(StyleGAN\_Bus)}
\end{minipage}
\begin{minipage}[t]{0.04\linewidth}
    \centering
    \rotatebox{90}{\scriptsize \hspace{0.5cm}(c)}
\end{minipage}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/feasibility/arch/aug0.png}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/feasibility/data/aug0.png}

\begin{minipage}[t]{0.04\linewidth}
    \centering
    \rotatebox{90}{\scriptsize \hspace{1cm}(d)}
\end{minipage}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/feasibility/arch/epoch15_all_f1_f2_aug.pdf}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/feasibility/data/epoch12_all_f1_f2_aug.pdf}

\vspace{-4pt}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{\scriptsize StyleGAN3 $\rightarrow$ StyleGAN2}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{\scriptsize StyleGAN\_Bus $\rightarrow$ StyleGAN\_Cat}
\end{minipage}
% \caption{\color{red}(a-b) Generated images by different models. (c) Output images by sending images from (a) to an augmentation model $A$. (d) Curves of averaged azimuthal integral spectrum calculated on images from (a-c). X-axis means a specific radius on the 2D spectrum (or spatial frequency intuitively), and y-axis represents sum of the spectrum magnitude of frequencies at this radius.}
% Send generated images from one model to an augmentation model $A$, the azimuthal integral spectrum could be converted to another model by the reconstruction residuals.}
\caption{(a) Images generated by the source model $M_{1}$. (b) Images generated by the respective target model $M_{2}$. (c) Feed images from source model $M_{1}$ to an augmentation model $A$ to simulate target model $M_{2}$'s trace while keeping the semantics unchanged. (d) Averaged azimuthal integral spectrum calculated on images from (a)-(c). X-axis means a specific radius on the 2D spectrum (or spatial frequency intuitively), and y-axis represents the sum of the spectrum magnitude of frequencies at this radius.}
\vspace{-5mm}
\label{fig:feasibility}
\end{figure}

 % (\eg, StyleGAN3 $\rightarrow$ StyleGAN2)

==> Figures/ft_seed_hist.tex <==
\begin{figure}[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=0.8\linewidth]{Images/ft_seed_hist3.pdf}
% \vspace{-4pt}
\caption{Confidence histograms on data from ProGAN\_celeba\_seed0, unseen seed model (ProGAN\_celeba\_seed1), and finetuned models (ProGAN\_celeba\_seed0\_finetuned).}
\vspace{-5mm}
\label{fig:ft_seed_hist}
\end{figure}

==> Figures/hist_compare.tex <==

% \newcommand\pecomparisonfigurewidth{0.48}
\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering
% \includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/hist/base-tsne.pdf}
% \includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/hist/POSE-d0.95-tsne.pdf}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/hist/base-hist.pdf}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/hist/POSE-hist-a0.95.pdf}
% \vspace{-4pt}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{(a) Base}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{(b) POSE}
\end{minipage}
% \caption{Feature space visualization (above) and confidence histograms (below) for base model and our proposed POSE.}
% \caption{Confidence histograms (below) for base model and our proposed POSE.}
\caption{Confidence histograms for base model and POSE.}
\label{fig:hist_compare}
\vspace{-5mm}
\end{figure}

==> Figures/hist_tsne.tex <==


\newcommand\casewidth{0.242}
\begin{figure}[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\casewidth\linewidth]{Images/case2/tsne-epoch29-case_base_celeba_ProGAN_seed0_celeba_MMDGAN.pdf}
\includegraphics[width=\casewidth\linewidth]{Images/case2/tsne-epoch29-case_base_stylegan3_cat_sngan_cat.pdf}
\includegraphics[width=\casewidth\linewidth]{Images/case2/tsne-epoch24-case_celeba_ProGAN_seed0_celeba_MMDGAN2.pdf}
\includegraphics[width=\casewidth\linewidth]{Images/case2/tsne-epoch24-case_stylegan3_cat_sngan_cat2.pdf}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/hist/base-hist.pdf}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{Images/hist/POSE-hist-a0.95.pdf}
% \vspace{-4pt}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{(a) Base}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{(b) POSE}
\end{minipage}
\caption{Feature space visualization (top) and confidence histograms (bottom) for Base method and our proposed POSE.}
% \caption{Confidence histograms (below) for base model and our proposed POSE.}
% \caption{Confidence histograms for base model and POSE.}
\label{fig:hist_tsne}
\vspace{-6mm}
\end{figure}

==> Figures/method.tex <==
% \begin{figure*}
% \begin{center}
% \includegraphics[width=0.8\linewidth]{Images/method7.png} 
% \end{center}
%   \caption{Overview of progressive open-space expansion.\fan{add spectral distribution for different images?}}
% \label{fig:method}
% \end{figure*}

% At each training iteration, a new augmentation model is trained and constrained to generate augmented data different from old augmented data.
\begin{figure*}[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=0.85\linewidth]{Images/method8.pdf} 
\caption{Overview of our proposed POSE. The open space is simulated by involving augmentation models progressively.}
\label{fig:method}
\vspace{-5mm}
\end{figure*}

==> Figures/method_feasibility.tex <==

\newcommand\methodwidth{0.68}
\newcommand\feasiwidth{0.3}

\begin{figure*}
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\feasiwidth\linewidth]{Images/method7.png}
\includegraphics[width=\methodwidth\linewidth]{Images/method7.png}
\vspace{-4pt}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{(a) Base}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{(b) POSE}
\end{minipage}
\caption{Confidence histograms for closed-set and unseen seed, unseen architecture, unseen dataset open-set samples.\wdd{Bigger font size in the lengends. For the scatter plot, please use the same color theme as Fig 5.}}
\vspace{-5mm}
\label{fig:method_feasibility}
\end{figure*}

==> Figures/progressive.tex <==

\begin{figure*}
\begin{center}
\includegraphics[width=0.8\linewidth]{Images/progressive.png} 
\end{center}
  \caption{Progressive training mechanism}
\label{fig:progressive}
\end{figure*}



==> Figures/robustness.tex <==

% \newcommand\diffusionsamplewidth{0.195}
\begin{figure*}[htbp]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/robustness/robust_blur.pdf}
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/robustness/robust_jpeg.pdf}
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/robustness/robust_light.pdf}
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/robustness/robust_noise.pdf}
\includegraphics[width=\diffusionsamplewidth\linewidth]{Images/robustness/robust_crop.pdf}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(a) Blurring}
\end{minipage}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(b) JPEG compression}
\end{minipage}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(c) Lighting}
\end{minipage}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(d) Noise}
\end{minipage}
\begin{minipage}[t]{\diffusionsamplewidth\linewidth}
    \centering
    \figtext{(e) Crop and resize}
\end{minipage}
\caption{Robustness analysis. The results are evaluated on Split 1 of the benchmark.}
\label{fig:robustness}
% \vspace{-5mm}
\end{figure*}

==> Figures/sim_matrix.tex <==

\begin{figure}
\begin{center}
\includegraphics[width=\linewidth]{Images/cm-compare.png}
\end{center}
  \caption{Similarity comparison}
\label{fig:method}
\end{figure}

==> Figures/task.tex <==
\begin{figure}[!t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\linewidth]{Images/intro9.png} 
\caption{Open-set model attribution problem: The unknown classes include unknown models different from known models in training seeds, architectures, or training datasets. The goal is to simultaneously attribute images to known models and identify those from unknown ones.}   
\label{fig:intro}
\vspace{-5mm}
\end{figure}


==> Figures/tsne_expansion.tex <==

% \begin{figure*}
% \begin{center}
% \includegraphics[width=0.99\linewidth]{Images/progressive_expansion.png} 
% \end{center}
%   \caption{TSNE of progressive open-space expansion.}
% \label{fig:method}
% \end{figure*}


\newcommand\biascomparisontextwidth{0.05}
\newcommand\biascomparisonfigurewidth{0.17}
\newcommand\legendwidth{0.93}

\begin{figure}
\setlength{\abovecaptionskip}{2mm}
\centering
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{POSE w/o $\mathcal{L}_{\text{div}}$}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/wo_div/prog-5-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/wo_div/prog-10-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/wo_div/prog-15-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/wo_div/prog-20-s1.pdf}
\end{minipage}
\begin{minipage}{0.21\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/all2_sim_matrix_wodiv.pdf}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{POSE}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/div_d0.95/prog-5-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/div_d0.95/prog-10-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/div_d0.95/prog-15-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/div_d0.95/prog-20-s1.pdf}
\end{minipage}
\begin{minipage}{0.21\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/all2_sim_matrix.pdf}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{}}
\end{minipage}
\begin{minipage}{\legendwidth\linewidth}
    \includegraphics[width=\linewidth]{Images/all2-prog/legend.pdf}
\end{minipage}

\vspace{4pt}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(a) N=5}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(b) N=10}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(c) N=15}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(d) N=20}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(e) Pairwise Similarity}
\end{minipage}
\caption{(a-d) Feature space visualization of progressive open space expansion process without (top) and with $\mathcal{L}_{\text{div}}$ (bottom). \textbf{\textcolor{KnownColor}{Blue}} triangles are data of one known class, and circles in other colors are augmented data for this class by different augmentation models. (e) Pairwise similarities of open space expanded by 20 augmentation models. Bluer color indicates higher similarity.} 
\vspace{-7mm}
\label{fig:tsne_expansion}
\end{figure}


==> Figures/tsne_expansion2.tex <==

\newcommand\biascomparisontextwidth{0.05}
\newcommand\biascomparisonfigurewidth{0.18}

\begin{figure}
\centering
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{POSE w/o $\mathcal{L}_{\text{div}}$}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/prog2/wo_div/prog-4-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/prog2/wo_div/prog-9-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/prog2/wo_div/prog-14-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/prog2/wo_div/prog-19-s1.pdf}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{Images/prog2/wo_div/wodiv-cm-all2.pdf}
% \end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{POSE}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/prog/div/prog-0-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/prog/div/prog-3-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/prog/div/prog-6-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/prog/div/prog-9-s1.pdf}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{Images/prog/div/cm-all2.pdf}
\end{minipage}

\vspace{4pt}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(a) K=1}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(b) K=4}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(c) K=7}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(d) K=10}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{(e) Pairwise Similarity}
\end{minipage}
\caption{tSNE of progressive open space expansion process.}
\vspace{-5mm}
\label{fig:tsne_expansion2}
\end{figure}


==> Sections/0_abstract.tex <==
%%%%%%%%% ABSTRACT
% 背景 -> 任务 -> 问题 -> 解决方法 -> 结果
% 重点：
% 1. 问题到解决方法的衔接
% 2. 解决方法和题目的衔扣
% \usepackage[colorlinks,linkcolor=blue]{hyperref}
\begin{abstract}

Despite the remarkable progress in generative technology, the Janus-faced issues of intellectual property protection and malicious content supervision have arisen. Efforts have been paid to manage synthetic images by attributing them to a set of potential source models. However, the closed-set classification setting limits the application in real-world scenarios for handling contents generated by arbitrary models. In this study, we focus on a challenging task, namely \textit{Open-Set Model Attribution} (OSMA), to simultaneously attribute images to known models and identify those from unknown ones. Compared to existing open-set recognition (OSR) tasks focusing on semantic novelty, OSMA is more challenging as the distinction between images from known and unknown models may only lie in visually imperceptible traces. To this end, we propose a \underline{P}rogressive \underline{O}pen \underline{S}pace \underline{E}xpansion (POSE) solution, which simulates open-set samples that maintain the same semantics as closed-set samples but embedded with different imperceptible traces. Guided by a diversity constraint, the open space is simulated progressively by a set of lightweight augmentation models. We consider three real-world scenarios and construct an OSMA benchmark dataset, including unknown models trained with different random seeds, architectures, and datasets from known ones. Extensive experiments on the dataset demonstrate POSE is superior to both existing model attribution methods and off-the-shelf OSR methods. Github: \href{https://github.com/TianyunYoung/POSE}{https://github.com/TianyunYoung/POSE}

\end{abstract}


% tailored for open-set model attribution, whose key idea is to
%    Model attribution aims to identify the source model of generated contents. 
%    Despite its potential benefits in intellectual property protection and malicious content supervision, most existing works are under closed set scenarios, which limits the use for identifying (handling) contents generated by unseen models.
%In this work, we present the first study on \textit{Open-Set Model Attribution} (OSMA) to simultaneously attribute images to known models and identify those from unknown ones. 



==> Sections/0_bak.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
    Model attribution aims to identify the source model of generated contents. 
    Despite its potential benefits in intellectual property protection and malicious content supervision, most existing works are under closed set scenarios, which limits the use for identifying (handling) contents generated by unseen models.
    In this work, we present the first study on \textit{Open-Set Model Attribution} (OSMA) to simultaneously attribute images to known models and identify those from unknown ones. 
    Different from existing open-set recognition (OSR) problems concentrating on semantic novelty, OSMA focuses on distinctions in visually imperceptible traces, which existing OSR methods could hardly handle. 
    We introduce a \underline{P}rogressive \underline{O}pen \underline{S}pace \underline{E}xpansion method (POSE) tailored for open-set model attribution, whose key idea is to simulate ``effective'' and ``diverse'' open-set samples via a progressive training mechanism. 
    For OSMA evaluation, we construct a benchmark considering three challenging open-set setups in real-world scenarios, which include unseen models with different training seeds, architecture, and datasets from seen models. 
    Extensive experiments on the benchmark demonstrate POSE is superior to both existing fake image attribution methods and OSR methods. 
\end{abstract}

==> Sections/1_bak.tex <==

%%%%%%%%% BODY TEXT
\section{Introduction}
\label{sec:intro}

Advanced generative modeling technology\fan{add references} can create extremely realistic visual content, which also becomes a sharp weapon for disinformation production. 
Severe impacts of maliciously generated content have motivated a plethora of work on the detection of generated images. 
However, with the rapid pace of generative technology, this may not be the end. 
% Model attribution, \ie, identify the source model of generated contents, has been paid attention to recently, which could assist law enforcers in tracing the producers of malicious content, as well as help to claim the ownership of copyrighted generative models. 
One the one hand, there is need to further trace the producers of malicious content. One the other hand, the ownership of a copyrighted generative models needs to be protected. To solve these problems, model attribution, \ie, identify the source model of generated contents, has been paid attention to recently. In this field, existing works~\cite{marra2019gans,yu2019attributing,frank2020leveraging,xuan2019scalable,yang2022aaai,bui2022repmix} have validated the existence of GAN fingerprints and showed the feasibility of attributing fake images to a fixed and finite set of models. However, most of them are limited to a closed-set setup, which is impractical in the real world scenario where exists an ever-growing number of unseen models. In this paper, we aim at the new problem of Open-Set Model Attribution (OSMA), i.e., simultaneously attribute images to known source models and identify those from unknown ones. 

\inputfigure{task}
An intuitive way for open-set recognition (OSR) is simulating the open set space. Among existing OSR works, mixup~\cite{zhou2021learning}, autoencoder~\cite{neal2018open}, and GAN~\cite{chen2021adversarial, kong2021opengan, moon2022difficulty} are employed to simulate open-set samples or features. Despite their success in tackling existing OSR problems, we argue that they are sub-optimal for the aforementioned open-set model attribution problem. On the one hand, generative models are leveraged to model the semantics of known classes~\cite{neal2018open, chen2021adversarial, kong2021opengan, moon2022difficulty}. For complex semantic simulation, generative models contain multiple convolution layers and more sophisticated generative results in better OSR performance~\cite{perera2020generative}. However, our task focuses on distinctions in visually imperceptible traces. On the other hand, there exists an ever-growing number of unseen models in open world. Simulated open samples or features by a single generator~\cite{kong2021opengan, chen2021adversarial, moon2022difficulty} or mechanism~\cite{zhou2021learning} are not diverse enough to reduce the open space risk. This is because a single generator can hardly model the boundary of multiple known classes on a disconnected manifold. 

% could exhaustively expand the open space. 
In this paper, we propose \textit{Progressive Open Space Expansion} (POSE) tailored for open-set model attribution. The goal is to simulate diverse open-set samples with unknown traces via s progressive training mechanism. 

Firstly, how can we generate samples with unknown low-level traces? Previous works have found the influence of architecture~\cite{yang2022aaai} and model weights~\cite{yu2019attributing} to GAN fingerprints. However, for unknown trace simulation, it's a daunting task to consider a large number of the architectures and model weights for all layers. Based on an empirical study, we found the weights of last convolution layer of generative models make up the main components of GAN fingerprints. Thus, we propose to employ multiple tiny convolution networks to simulate unknown traces, which reconstruct the content of known images with small residuals, modifying traces of known classes with subtle and diverse perturbations. Our further analysis proves the feasibility of utilizing these networks to model rich unknown traces. 

To guarantee the diversity of the generated samples, we employ multiple generators. However, naively using multiple generators may lead to a trivial solution where all generators generate images with similar traces. To avoid this, we propose a novel progressive training mechanism to span the open space iteratively. By a diversity objective, we ensure that the open samples generated by the next generator should vary largely from the samples generated by the previous generators, and be close to the known classes in the embedding space learned on all the existing samples. As such, the next generator will simulate open samples in the unexplored open space along the boundary of the known distribution. 

% Previous works have found that, with architecture and dataset fixed, GAN models trained with different seeds have different fingerprints, indicating model weights leaves fingerprints. GAN architecture
% Secondly, how can we ensure the generated samples lie around the boundary of known classes, i.e., neither too far nor too close to the known distribution as aforementioned? We surprisingly observe that the effectiveness of generated open samples is closely related to the closed-set classification accuracy. Thus, we define the boundary of the known distribution by the mean squared error lower-bound between the generated open-set samples and the known images that have the maximum closed-set classification accuracy.

Our contributions can be summarized as follows:
\begin{itemize}
    \item To tackle an important challenge when applying model attribution to real-world scenarios, we are the first to raise a new issue, the open-set model attribution, which simultaneously attributes images to known models and identifies images from unknown models. 
    \item We present a novel method named POSE to generate diverse open-set samples with unknown traces via a progressive training mechanism. 
    \item To validate the effectiveness of our method, we build a large benchmark to simulate real world model attribution scenarios, including seen real, seen fake, unseen real and unseen fake. Extensive experiments on the benchmark prove that POSE is superior than not only existing fake image attribution methods but also OSR methods.  
\end{itemize}
\fan{TLTD}


==> Sections/1_intro.tex <==

%%%%%%%%% BODY TEXT
\section{Introduction}
\label{sec:intro}
Advanced generative modeling technology can create extremely realistic visual content, leading to dramatic changes in the field of AI-enhanced design, arts, and meta-universe~\cite{karras2021alias,rombach2021highresolution,wang2023towards}.
Whereas, the broadcasting of malicious content generated by open source generation models has brought severe social impacts~\cite{deepfake1,deepfake2,deepfake3}. Furthermore, new challenges have arisen for the ownership protection of copyrighted digital generative models. To solve these problems, model attribution, \ie, identifying the source model of generated contents, has drawn increasing attention recently~\cite{marra2019gans,yu2019attributing,xuan2019scalable,yang2022aaai,bui2022repmix}. 
\inputfigure{task}

Marra~\etal~\cite{marra2019gans} are among the first to point out that GAN models leave specific fingerprints in the generated images, just like camera devices.
Further researches~\cite{yu2019attributing,frank2020leveraging,xuan2019scalable,yang2022aaai,bui2022repmix} validate the existence of GAN fingerprints and show the feasibility of attributing fake images to a fixed and finite set of known models. However, most of these works focus on finding discriminative fingerprints among the contents generated by different GAN models following a simple closed-set setup. The ever-growing number of unseen source models in the real-world scenario appeal for a more generic approach. In this paper, we focus on the problem of Open-Set Model Attribution (OSMA), \ie, simultaneously attributing images to known source models and identifying those from unknown ones. 

An intuitive way to solve OSMA is to apply off-the-shelf open-set recognition (OSR) approaches to closed-set model attribution classifiers. Traditional OSR methods leverage the output logits to either reject or categorize the input images~\cite{bendale2016towards,shu2017doc}. However, following the discriminative line, the performance highly depends on the closed-set classifier~\cite{vaze2022openset}. The learned feature space is not rectified for open-set samples. Another mainstream of OSR methods is based on simulating open-set samples or features ~\cite{zhou2021learning,neal2018open,chen2021adversarial, kong2021opengan, moon2022difficulty}. By the simulation of open space, the learned feature space is more compact for closed-set categories ~\cite{zhou2021learning}, leading the detection of unknown samples more valid. Nevertheless, existing works only leverage a single generator~\cite{kong2021opengan, chen2021adversarial, moon2022difficulty} or mechanism~\cite{zhou2021learning} for simulating open-set samples or features, which are not diverse enough to reduce the open space risk for OSMA. A generator could produce open-set samples of different semantics, but its fingerprint is fixed and thus not suitable for the expansion of open space.

In this study, we propose \textit{Progressive Open Space Expansion} (POSE) tailored for open-set model attribution, which simulates the potential open space of challenging unknown models through involving a set of augmentation models progressively. For augmentation model construction, it can be daunting to consider all types of unknown models with a variety of architectures. Instead, lightweight networks composed of a few convolution layers are employed. They serve as “virtual” follow-up blocks of known models, augmenting closed-set samples to open-set samples surrounding them by modifying their fingerprints with reconstruction residuals. Despite the simple structure, these augmentation models show the potential to model traces of a variety of unknown models. To enrich the simulated open space, multiple augmentation models are involved. Instead of training them independently, we design a progressive training mechanism to ensure the diversity of simulated open space across models in a computation-effective way.

To validate the effectiveness of POSE in the open world, we construct a benchmark dataset considering three challenging unknown scenarios as shown in Figure~\ref{fig:intro}, which includes unknown models trained with either a different random seed, architecture or dataset from known models. Extensive experiments on the benchmark demonstrate POSE is superior to both existing GAN attribution methods and OSR methods. In summary, our contributions are:

% 没有得到这个结论
% Based on the discovery that shallow convolutional networks can simulate images with unseen model traces, 
\noindent $\bullet$ We tackle an important challenge for applying model attribution to open scenarios, the open-set model attribution problem, which attributes images to known models and identifies images from unknown ones. \\
\noindent $\bullet$ We propose a novel solution named POSE, which simulates the potential open space of unknown models progressively by a set of lightweight augmentation models, and consequently reduces open space risk. \\
\noindent $\bullet$ We construct an OSMA benchmark simulating the real-world scenarios, on which extensive experiments prove the superiority of POSE compared with existing GAN attribution methods and off-the-shelf OSR methods. 


==> Sections/2_bak.tex <==
\section{Related Work}

\noindent\textbf{Open-Set Recognition.} T


he problem of open-set recognition (OSR) aims at recognizing known classes and rejecting unknown classes simultaneously. Existing works addressing the OSR problem mainly follow two lines: discriminative perspective and generative perspectives. 

From the discriminative perspective, many efforts have been made to adapt traditional discriminative models to the OSR problem, including works on Support Vector Machine (SVM)~\cite{scheirer2012toward, scherreik2016open, scheirer2014probability, jain2014multi}, sparse representation-based classifier~\cite{zhang2016sparse}, distance-based classifier~\cite{bendale2015towards, mendes2017nearest}, and margin distribution-based classifier~\cite{rudd2017extreme, vignotto2018extreme}, etc. Recently, Deep Neural Networks (DNN) are used in various fields owing to the excellent representation ability. Most DNN classifiers follow a typical softmax cross-entropy loss, which often leads to unreasonable high confidence on unknown samples. To solve this, Openmax~\cite{bendale2016towards} based on the Extreme Value Theory (EVT) replaces softmax for fooling/rubbish and unrelated open set images, and K-sigmoid~\cite{shu2017doc} conducted score analysis to search for threshold. 

From the generative perspective, existing works fall into two categories: 1) Employing generative models to model known-class representation~\cite{oza2019c2ae, sun2020conditional, zhang2020hybrid, guo2021conditional, perera2020generative, yoshihashi2019classification}. 2) Generating unknown samples to simulate the open space~\cite{ge2017generative, neal2018open, chen2020learning, zhou2021learning, chen2021adversarial, kong2021opengan, moon2022difficulty}. Our method falls into the second category. For this category, G-openmax~\cite{ge2017generative} improved openmax~\cite{bendale2016towards} via generating extra images to represent the unknown class. OSRCI~\cite{neal2018open} developed encoder-decoder GAN architecture to generate counterfactual examples. ARPL~\cite{chen2021adversarial} improved prototype learning~\cite{chen2020learning} by generating fake images with GAN. PROSER~\cite{zhou2021learning} simulated the open space between class boundaries based on manifold mixup~\cite{verma2019manifold}. OpenGAN~\cite{kong2021opengan} utilized GAN's discriminator as the open-set likelihood function. DIAS~\cite{moon2022difficulty} generate fakes with diverse difficulty levels by GAN and Copycat network. These proposed OSR methods mainly focuses on semantic novelty, which are sub-optimal for our problem concentrating on differences in low-level traces. 



\noindent \textbf{Model Attribution.} Model attribution for generated images could be classified into positive attribution~\cite{kim2020decentralized,yu2020artificial,yu2020responsible} and passive attribution~\cite{marra2019gans,yu2019attributing,frank2020leveraging,joslin2020attributing,xuan2019scalable,bui2022repmix,yang2022aaai,girish2021towards}. Works on positive attribution insert artificial fingerprints~\cite{yu2020artificial,yu2020responsible} or keys ~\cite{kim2020decentralized} directly into the generative model. The fingerprint or key can be decoupled from generated images to trace the source model. Positive attribution requires ``white-box" generative model training and thus is limited in ``black-box" scenarios when only generated images are available. What is more, positive attribution methods need to modify the model with source information, which cannot handle already trained models and may reduce the generation quality. Thus, we solve fake image attribution under the passive setting. 

Passive attribution aims at identifying the intrinsic differences between different types of generated images without getting access to the generative model. The work in~\cite{marra2019gans} used averaged noise residual to represent GAN fingerprint. The work in~\cite{yu2019attributing} took the final classifier features and reconstruction residual as the image fingerprint. The work in~\cite{frank2020leveraging} observed the discrepant DCT frequency spectrums exhibited by images generated from different GAN architectures, and then used the DCT frequency spectrum for source identification. The work in~\cite{joslin2020attributing} derived a similarity metric on the frequency domain for GAN attribution. To expand the application scenario, DNA-Det~\cite{yang2022aaai} and RepMix~\cite{bui2022repmix} moved a step further from model attribution to architecture attribution. However, they still cannot deal with unseen architectures. Girish et al. ~\cite{girish2021towards} pioneer to propose an iterative pipeline to attribute images to known sources as well as discovering unknown sources. However, this work only provided a general pipeline suitable for common classification tasks and only considered unseen models trained with different architectures, neglecting the inherent challenges in open-set model attribution. Our proposed POSE is tailored for open-set model attribution, and considered more situations in open-world such as model fine-tuning, different random seeds and unseen datasets.

% research gap

==> Sections/2_related.tex <==
\section{Related Work}
% research gap
\noindent\textbf{Open-Set Recognition.} Works on open-set recognition mainly follow a discriminative or generative line. The typical routine from the discriminative perspective first trains a K-way classifier on the closed set and then calibrates the confidence to a reasonable distribution for open-set dicrimination~\cite{bendale2016towards, shu2017doc}. However, without rectification to the feature space, the performance depends heavily on the closed-set classifier~\cite{vaze2022openset}. Generative-based approaches employ generative models for two purposes: 1) to threshold the test-time reconstruction error as an open-set indicator~\cite{oza2019c2ae, sun2020conditional, zhang2020hybrid, guo2021conditional, perera2020generative, yoshihashi2019classification}, or 2) to simulate the potential open space for augmenting classifier training~\cite{ge2017generative, neal2018open, chen2020learning, zhou2021learning, chen2021adversarial, kong2021opengan, moon2022difficulty}. For the open-set model attribution problem, it is sub-optimal to follow the reconstruction approach, as the intrinsic differences between samples generated by known and unknown models mainly lie in visually imperceptible traces, which are too subtle to be thresholded. For the second line, mixup mechanism~\cite{zhou2021learning}, GAN~\cite{chen2021adversarial, kong2021opengan, moon2022difficulty}, and auto-encoder~\cite{neal2018open} are leveraged for open space simulation. However, the open space risk for OSMA could be hardly reduced by a single generator or mechanism. The generators are proposed to generate images with different semantics, unable to produce diverse open-set fingerprints by its fixed weights and architecture. In this study, we simulate a rich open space for potential unknown models by involving a set of augmentation models progressively, and reduce the open space risk better.

\noindent \textbf{Model Attribution.} Model attribution aims to identify the source model of generated contents. Existing works tackle model attribution through an active~\cite{kim2020decentralized,yu2020artificial,yu2020responsible} or passive manner~\cite{marra2019gans,yu2019attributing,frank2020leveraging,joslin2020attributing,xuan2019scalable,yang2021learning,girish2021towards}. 
Active methods embed artificial fingerprints~\cite{yu2020artificial,yu2020responsible} or keys~\cite{kim2020decentralized} into the generative model during the training process and then decouple them for source attribution in testing. Despite their capability of protecting particular models, requiring access to the training process limits their application in handling fake images generated by arbitrary models. With the verification of the existence of GAN fingerprints~\cite{marra2019gans,yu2019attributing}, passive model attribution methods~\cite{marra2019gans,yu2019attributing,frank2020leveraging,joslin2020attributing,xuan2019scalable,girish2021towards,yang2021learning} are proposed by capturing the intrinsic differences in GAN fingerprints. Typically, a classifier is trained to distinguish images generated from a fixed and finite set of models, yet not applicable in the real world of an ever-growing number of unknown models. Some works, like DNA-Det~\cite{yang2022aaai} and RepMix~\cite{bui2022repmix}, attempt to expand the application scenarios to identify images from unknown models of known architectures by relaxing the attribute objective to the model architecture instead of a specific model. Though more generic compared with closed-set model attribution, architecture-level attribution still does not consider unknown models with unseen architectures. Girish~\etal~\cite{girish2021towards} pioneers to consider open-world GAN attribution and discovery. However, the proposed approach follows a general semi-supervised learning pipeline, overlooking the intrinsic challenge of imperceptible trace discrimination. Our proposed POSE is tailored for the trace discrimination challenge and achieves better performance in not only open-set model attribution but also unknown model clustering. 


==> Sections/3_bak.tex <==

\section{Method}

We aim at the problem of open-set model attribution: to attribute an image to its source model of known classes while simultaneously recognizing images from unknown models. To solve the problem, we propose Progressive Open Space Expansion (POSE). Let $\delta\mathcal{Z}$ be the boundary of the embedding space $\mathcal{Z}$ of the known classes. $\mathcal{O}_{i}$ is the spanned open space by $i$-th augmentation model. The goal of POSE to simulate $\delta\mathcal{Z}$ exhaustively by the combination of $\mathcal{O}_{i}$:
\begin{equation}
\bigcup_{i}\mathcal{O}_{i} \rightarrow \delta\mathcal{Z} \label{goal}.
\end{equation}

To achieve this goal, two objectives should be satisfied:
\begin{itemize}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
\item \textbf{Efficiency objective}: to delineate the boundary of the known space, the generated open-set samples should be close to the known samples but with different imperceptible generator fingerprints.
%the generated open space should lie on the boundary of known space, such that the generated samples are effective enough to improve the performance on challenging open-set samples.
\item \textbf{Diversity objective}: the generated open space by different generators should vary from each other, such that $\delta Z$ could be simulated as large as possible.
\end{itemize}
Formally, we have the following objective functions respect to the above two objectives: 
\begin{equation}
\text{To satisfy efficiency:} \max \mathcal{O}_{i} \cap \delta\mathcal{Z} \label{eff},
\end{equation}
\begin{equation}
\text{To satisfy diversity:} \min \mathcal{O}_{i} \cap \mathcal{O}_{j}, i \ne j. \label{div}
\end{equation}

Next, we describe the POSE framework and how to stimulate the open space by satisfying the two objectives.


% 原理（验证的假设） -> 方法 -> 方法的可行性
\subsection{Augmentation Model Construction}
\label{sec:m0}

% In traditional generative-based OSR methods, generative models are trained to model semantics and more sophisticated generative models result in better performance~\cite{perera2020generative}. However, the training process of generative models is resource-consuming. Different from OSR methods focusing on semantic novelty, open-set model attribution concentrates more on differences in low-level traces. Without semantics modeling requirements, we generate open samples by tiny auto-encoders with only two convolution layers. 

% 是否有可能只用简单的参数量少的网络去模拟未知的模型
% To verify this assumption, we design an empirical study as follows:

When simulating the open-space of generative models, it is daunting to sample a large amount of unknown architectures with different combinations of layers, or to sample unknown models with different weights in all parameters. To simplify the problem, we question whether it is possible to simulate rich open space using tiny networks with few layers, such that the simulated open space could be greatly reduced. Luckily, as discussed in \cite{chandrasegaran2021closer} and \cite{karras2021alias}, the frequency content of the outputs of individual layers are limited by the sampling resolution of the corresponding outputs based on Sampling Theorem~\cite{jain1989fundamentals}. Thus, GAN fingerprints is likely to be most correlated to the last few layers of generative models. To produce unknown traces similar to known classes. Augmented images should lie on similar frequency band to known classes. As such, the augmentation model should not contain upsampling layers, which would heavily influence high frequency components. Convolution weights are responsible for modifying the frequencies, and different kernel weights introduces diverse traces. As a result, we propose to use a tiny networks of convolution layers as augmentation models. 

\noindent \textbf{Feasibility of tiny network to model unknown traces:}
In real world, there exist a large number of unknown models with diverse traces. Considering the simple structure of augmentation models, we further testify the feasibility of them to model traces of unknown models with different training seed, architecture and dataset, respectively. 

Suppose the known model is a StyleGAN3 model trained on FFHQ, we testify whether there exists an augmentation model $A$ that could modify the frequency distribution of it to a unknown StyleGAN2 model trained on FFHQ. We propose to train the augmentation model with a $\mathcal{L}_{\text{spectral}}$:
\begin{equation}
    \mathcal{L}_{\text{spectral}} = \|\mathbf{x} - A(\mathbf{x})\| + \lambda \|\text{Freq}(A(\mathbf{x}_{1})) - \text{Freq}(\mathbf{x}_{2})\|,
\end{equation}
where $\lambda$ is a hyper-parameter that balance pixel reconstruction loss and frequency modification loss.  $\text{Freq}()$ is the azimuthal integration~\cite{durall2020watch} measuring the averaged spectral distribution of images. 
As shown in Figure~\ref{fig:feasibility}, through the optimization of $\mathcal{L}_{\text{spectral}}$, we can find an augmentation model able to transform frequency distribution of a StyleGAN3\_FFHQ model to a Style2\_FFHQ model, and a StyleGAN\_Bus model to a StyleGAN\_Cat model with little distortion in pixel. 

\inputfigure{feasibility}
\subsection{Progressive Open Space Expansion}
\label{sec:m1}

Fig.~\ref{fig:method} shows the framework of POSE. Our model consists of task models and augmentation models. The task models consist of a feature extractor $F: \mathcal{X} \rightarrow \mathcal{Z}$ mapping images from the input space to the embedding space, and a classification head $H: \mathcal{Z} \rightarrow \mathcal{Y}$ mapping the embedding space to the label space. The augmentation models convert the input image $\mathbf{x}$ to augmented image $\tilde{\mathbf{x}}$ whose embedding space $\tilde{\mathcal{Z}}$ is on the boundary of $\mathcal{Z}$. The progressive training progress trains augmentation models one at a time.

\noindent \textbf{Training task models:} The overall loss function for task models is formulated as follows:
\begin{equation}
    \mathcal{L}_{\text{task}} = \mathcal{L}_{\text{cls}}(\mathbf{x}) + \alpha \mathcal{L}_{\text{metric}}(\mathbf{x},\tilde{\mathbf{x}}),
\end{equation}
where $\mathcal{L}_{\text{cls}}$ is the classification loss calculated on input image $\mathbf{x}$ defined in Eq.~\eqref{cls}, and $\mathcal{L}_{\text{metric}}$ is a metric loss calculated on the embedding of both input image $\mathbf{x}$ and augmented image $\tilde{\mathbf{x}}$ defined in Eq.~\eqref{metric}. $\alpha$ is a hyper-parameter.

Specifically, $\mathcal{L}_{\text{cls}}$ is a cross-entropy loss for known class: 
\begin{equation}
    \mathcal{L}_{\text{cls}}(\mathbf{y}, \hat{\mathbf{y}})=-\sum_i y_i \log \left(\hat{y}_i\right) \label{cls},
\end{equation}
where $\hat{\mathbf{y}}$ is the \textit{softmax} output of the classification head; $\mathbf{y}$ is the one-hot vector representing the ground truth class of $\mathbf{x}$; $y_{i}$ and $\hat{y_{i}}$ represent the $i$-th dimension of $\mathbf{y}$ and $\hat{\mathbf{y}}$, respectively. 

$\mathcal{L}_{\text{metric}}$ is a triplet loss to distinguish the embedding of augmented data from input data, and simultaneously separating different known classes and augmented classes. For an input image $x_{i}$ with class $i$, we assign the augmented image by sending it into an augmented model to a new class label $i+C$, where $C$ is the total number of known classes, getting 2$C$ classes for all input and augmented data. Let $\bar{\mathcal{X}}=\mathcal{X}\cup\tilde{\mathcal{X}}$ be the combination of input and augmented data, and $\mathcal{T}_{z}=(\bar{x}_{a}^{z},\bar{x}_{b}^{z},\bar{x}_{n}^{z})$ be one of the triplet set $\mathcal{T}$ sampled from $\bar{\mathcal{X}}$, the triplet loss is calculated as follows:
\begin{equation}
    \mathcal{L}_{\text{metric}} = \sum_{\mathcal{T}_{z} \in \mathcal{T}} [\|\bar{x}^{z}_{a} - \bar{x}^{z}_{p}\|^{2}-\|\bar{x}^{z}_{a}-\bar{x}^z_{n}\|^{2}+ m]_{+} \label{metric},
\end{equation}
where $[\cdot]_{+}=\max(0,\cdot)$ denotes the hinge loss function, and $m$ is the violate margin that requires the distance of negative pairs to be larger than the distance of positive pairs, by at least a margin $m$. 

\noindent \textbf{Training augmentation models:} Let $\tilde{\mathbf{x}}_{p}$ be the augment image generated by present augmentation model, and $\tilde{\mathbf{x}}_{o}$ is generated by previous augmentation models. The overall loss function for present augmentation model is as follows:
\begin{equation}
    \mathcal{L}_{\text{aug}} = \mathcal{L}_{\text{recons}}(\mathbf{x},\tilde{\mathbf{x}}_{p}) + \beta \mathcal{L}_{\text{eff}}(\mathbf{x}, \tilde{\mathbf{x}}_{p}) + \gamma \mathcal{L}_{\text{div}}(\tilde{\mathbf{x}}_{o},\tilde{\mathbf{x}}_{p}),
\end{equation}
where $\mathcal{L}_{\text{recons}}$ is the reconstruction loss between augmented and input image in the pixel space, $\mathcal{L}_{\text{eff}}$ is the efficiency objective for satisfying Eq.~\eqref{eff}, and $\mathcal{L}_{\text{div}}$ is the diversity objective for satisfying Eq.~\eqref{div}. $\beta$ and $\gamma$ are two hyper-parameters. The implementations of $\mathcal{L}_{\text{div}}$ and $\mathcal{L}_{\text{eff}}$ are discussed in Sec.~\ref{sec:m2}.

\subsection{Efficiency and Diversity Objectives}
\label{sec:m2}
% Fig.~\ref{fig:progressive} shows the function of efficiency and diversity objective.
% \noindent\textbf{Efficiency Objective:}
\paragraph{Efficiency Objective}
The efficiency objective guarantees the generated open space should lie on the boundary of known space.
In other words, the generated open space should be as close as possible to the known space, but don't overlap with it. To achieve this, we apply a hinge reconstruction loss:
\begin{equation}
    \mathcal{L}_{\text{eff}} = \max(\epsilon,\|A(\mathbf{x}) - \mathbf{x}\|),
\end{equation}
where $A$ is the present augmentation model. $\epsilon$ is a lower bound for the reconstruction error. The augmentation model aims to generate images with similar semantics but different traces. It would be trivial if an extreme case happened when the model completely reconstructs the input image without error. thus we apply a lower bound for reconstruction to avoid such a situation.

\noindent\textbf{Further Discussion:} For model attribution, there exist two hard cases near the known space boundary, \textit{i.e.}, models trained with only seed different, and models fine-tuned from the known models. Following the discussion in ~\cite{lukas2019deep, li2021novel, pan2022metav}, the former should be regarded as different classes as they are trained independently, and the latter should still be regarded as known classes as fine-tuning could be taken as a transformation of the original model. Luckily, open-set samples generated by our augmentation models naturally lies in between the two cases. 

% \noindent\textbf{Diversity Constraint:} 
\paragraph{Diversity Objective}
Single augmentation model could only simulate one kind of trace similar to known models, which is insufficient for open space imitation. An intuitive way is to increase the number of augmentation models. However, as shown in Fig.~\ref{fig:tsne_wodiv}(a), naively 
increasing the number of augmentation models by training more models with different training seeds doesn't expand much open space, as they are quite similar in the embedding space. Thus, we expect the augmented space by different augmentation models should vary from each other, such that the boundary open space could be spanned as large as possible. 

We increase the diversity by a progressive training mechanism. When training the next augmentation model, we randomly select a previously trained augmentation model, and measure their distance in the embedding space of their generated images. We expect the distance could be large. However, simply increase the distance without direction would produce useless samples also far from the known classes. Hence, we apply an additional regularization between the embedding distance of augmented images and input images, to increase the diversity of augmentation models by optimizing toward an efficient direction.
\begin{equation}
    \mathcal{L}_{\text{div}} = - \|\tilde{\mathbf{z}}_{p} - \tilde{\mathbf{z}}_{o}\| + \|\tilde{\mathbf{z}}_{p} - \tilde{\mathbf{z}}\|.
\end{equation}

\noindent\textbf{Further Discussion:} 

\subsection{Overall Training Progress}

\renewcommand{\algorithmicrequire}{\textbf{Input:}} 
\renewcommand{\algorithmicensure}{\textbf{Output:}} 
\begin{algorithm}[h]
  \caption{The proposed Progressive Open-Space Expansion (POSE)}
  \label{alg::pose}
  \begin{algorithmic}[1]
    \Require
      Image of known classes $\mathbf{x}$; 
      Number of training epochs $N$
    \Ensure
      Learned task model $M$; 
      Learned augmentation models $\{A_{i}\}_{i=0}^{N-1}$
    \For{$i = 0, \dots, N$} 
        \If{$i=0$}
            \State Generate augment image $\tilde{\mathbf{x}}_{p}$ using $A_{0}$
            \State Train augmentation model $A_{0}$ using $\mathcal{L_{\text{eff}}}(\mathbf{x},\tilde{\mathbf{x}}_{p})$
        \Else
            \State Randomly select a previously trained augmentation model, and generate augment image $\tilde{\mathbf{x}}_{o}$
            \State Generate augment image $\tilde{\mathbf{x}}_{p}$ using $A_{i}$
            \State Train augmentation model $A_{i}$ using $\mathcal{L_{\text{eff}}}(\mathbf{x},\tilde{\mathbf{x}}_{p})$ and $\mathcal{L_{\text{div}}}(\tilde{\mathbf{x}}_{o},\tilde{\mathbf{x}}_{p})$
        \EndIf
        \State Generate augment image $\tilde{\mathbf{x}}_{p}$ using $A_{i}$
        \State Train task model $M$ using $\mathcal{L_{\text{task}}}(\mathbf{x},\tilde{\mathbf{x}}_{p})$
    \EndFor
  \end{algorithmic}
\end{algorithm}

\noindent \textbf{Recognizing unknown classes:} 
Given an input test image, we feed it into the feature extractor $F$ and classification head $H$. After a $\textit{softmax}$ function, we get predicted confidence scores for each class. If the max confidence score is larger than a threshold $\theta$, the image is recognized as the known category corresponding to the index of the score. Otherwise, it is detected as unknown.


==> Sections/3_method.tex <==

\section{Method}
We tackle the OSMA problem by simulating the potential open space of unknown models around the boundary of known space through a set of augmentation models. At a high level, for open space simulation, two key components are 1) the simulation tool, \ie, how to construct the augmentation models, as it determines the scope of open space that could be expanded, and 2) the expansion mechanism. Given the augmentation models, the expansion mechanism decides how to increase the number of them to expand the open space in an efficient direction. In the following, we describe the simulation tool (Section~\ref{sec:m0}) and expansion mechanism (Section~\ref{sec:m1}) in detail. 

\subsection{Augmentation Model Construction}
\label{sec:m0}
To simulate the space of unknown models, an intuitive way is to train a number of augmentation models approximating real unknown models. However, it is daunting to consider all types of unknown models of a variety of architectures. 
% We notice the discussion in~\cite{chandrasegaran2021closer} that the frequency bandwidth in generated images is largely determined by the spatial resolution, thus the few layers after the last upsampling layer are likely to contribute most to traces in the half-extended high-frequency band by the last upsampling layer, and there is hope to simulate a fair amount of the components of unknown model traces with tiny networks. 
Empirically, we construct the augmentation models as lightweight networks by optimizing a reconstruction loss. Severing as ``virtual" follow-up blocks of known models, augmentation models receive images from known models, maintain their semantics but modify the traces with reconstruction residuals. In this way, the augmented images would carry hybrid fingerprints of known classes and augmentation models as shown in Figure~\ref{fig:method}(b). 

For the specific architecture choice, the candidate layer components could be upsampling and convolution. Upsampling layer would heavily influence high frequencies~\cite{chandrasegaran2021closer} and produce trivial open-set samples, which is thus not ideal to be included. As shown in \cite{frank2020leveraging}, distinctions in GAN fingerprints exist in the frequency components. Equipped with rich learnable kernels, convolution layers are capable of modifying the frequencies, either suppressing or amplifying frequencies flexibly depending on the optimization objective~\cite{chandrasegaran2021closer}. Besides, \cite{yu2020responsible} achieves GAN network fingerprinting by modulating convolution weights with a 128-bit fingerprint, reaching a capacity of around $10^{36}$ fingerprinted models in principle. Given these works suggesting the effect of convolution layers on GAN fingerprints, we use tiny networks with two convolution layers as augmentation models. Detailed ablation study is in Section~\ref{sec:ablation}.
\inputfigure{feasibility}
\inputfigure{method}
\noindent \textbf{Feasibility of tiny networks to simulate unknown model traces.} It is non-trivial to measure the scope of open space that could be expanded. Motivated by existing work~\cite{frank2020leveraging} showing that frequency spectrum contains much information about model fingerprints, we adopt a simple but characteristic 1D representation of the Fourier power spectrum, azimuthal integration (AI) over the power spectrum~\cite{durall2020watch}, as a hand-crafted criterion for the fingerprint space. 
% {\color{red}Suppose $M_{1}$ is a known model and $M_{2}$ is a potential unknown model, to testify whether there exists an augmentation model $A$ able to expand the open space around model $M_{1}$ to cover model $M_{2}$ according to the criterion, $\mathcal{L}_{\text{spectral}}$ is optimized to modify the azimuthal integral spectrum of images from model $M_{1}$ to model $M_{2}$:}
Suppose $M_{1}$ is a known model and $M_{2}$ is a potential unknown model, to testify whether there exists an augmentation model $A$ able to expand the open space around model $M_{1}$ to cover model $M_{2}$ according to the criterion, $\mathcal{L}_{\text{spectral}}$ is optimized as follows:
\begin{equation}
    \mathcal{L}_{\text{spectral}}(\theta) = \|\mathbf{x} - A(\mathbf{x})\| + \lambda \|\text{Freq}(A(\mathbf{x}_{1})) - \text{Freq}(\mathbf{x}_{2})\|,
\end{equation}
where $\theta$ is the parameters of $A$. $\mathbf{x}_{1}$, $\mathbf{x}_{2}$ and $\mathbf{x}$ are images generated by model $M_{1}$, model $M_{2}$, and all images. $\text{Freq}(\cdot)$ is spectrum azimuthal integration. $\lambda$ is to balance two parts of $\mathcal{L}_{\text{spectral}}$. The first part is a pixel reconstruction loss constraining the reconstruction residual, and the second part is calculated in the frequency domain, converting the azimuthal integral spectrum of model $A$ to model $B$. 

As shown in Figure~\ref{fig:feasibility}, by optimizing $\mathcal{L}_{\text{spectral}}$, augmentation models are able to transform the spectrum of one model to another model of different architecture (\eg, StyleGAN3 $\rightarrow$ StyleGAN2) or of different training dataset (\eg, StyleGAN\_Bus $\rightarrow$ StyleGAN\_Cat) with visually imperceptible traces. These results suggest the potential of lightweight networks to simulate rich unknown traces. We also emphasize that unknown models are actually out of access in the real world. Our solution is to utilize a set of augmentation models to cover as much open space of potential unknown models as possible around the boundary of known space through a progressive training manner, which is described in Section~\ref{sec:m1}.
\vspace{-1mm}

\subsection{Progressive Open Space Expansion}
\label{sec:m1}

Figure~\ref{fig:method} shows the framework of POSE. Our model consists of a task model and $N$ augmentation models progressively involved. The task model $M$ conducts open-set recognition task, including a feature extractor $F: \mathcal{X} \rightarrow \mathcal{Z}$ mapping images from the input space to the embedding space, and a classification head $H: \mathcal{Z} \rightarrow \mathcal{Y}$ for $K$-way known class classification, where $K$ is the number of known classes. The augmentation models $\{A_{i}\}^{N-1}_{0}$ are trained progressively one at an epoch, simulating the open space by converting input images $\mathbf{x}$ to augmented images $\tilde{\mathbf{x}}$. 

\noindent \textbf{Training augmentation models.} Let $\tilde{\mathbf{x}}_{\text{new}}$ be the augmented images generated by the present augmentation model (with a solid edge), and $\tilde{\mathbf{x}}_{\text{old}}$ is generated by a randomly selected old augmentation model (with a dashed edge). The overall loss function for the present augmentation model is as follows:
\begin{equation}
    \mathcal{L}_{\text{aug}} = \mathcal{L}_{\text{recons}}(\mathbf{x},\tilde{\mathbf{x}}_{\text{new}}) + \mathcal{L}_{\text{div}}(\tilde{\mathbf{x}}_{\text{old}},\tilde{\mathbf{x}}_{\text{new}}),
\end{equation}
where $\mathcal{L}_{\text{recons}}$ is a reconstruction loss between augmented and input images in the pixel space, and $\mathcal{L}_{\text{div}}$ is a diversity constraint to enlarge the difference between new and old augmented data in the embedding space.

To expand the simulated open space, an intuitive way is to increase the number of augmentation models. However, naively increasing the number of augmentation models by training them independently could result in similar simulated open space across models as shown in Figure~\ref{fig:tsne_expansion}(top). Thus, we propose to increase the diversity progressively by constraining the discrepancy of old and new augmented data at each iteration. Simply increasing the embedding distance of $\tilde{\mathbf{x}}_\text{{new}}$ and $\tilde{\mathbf{x}}_\text{{old}}$ without direction would produce trivial samples also far from the known data. Hence, we apply a regularization term narrowing the embedding  between new augmented images $\tilde{\mathbf{x}}_\text{{new}}$ and known images $\mathbf{x}$, to increase the diversity towards a direction approaching the known space:
\begin{equation}
    \mathcal{L}_{\text{div}} = \alpha F_{cos}(\tilde{\mathbf{z}}_{\text{new}},\tilde{\mathbf{z}}_{\text{old}}) - \beta \min(F_{cos}(\tilde{\mathbf{z}}_{\text{new}}, \mathbf{z}), d),
    \label{div}
\end{equation}
% \begin{equation}
%     \mathcal{L}_{\text{div}} = \alpha F_{cos}(\tilde{\mathbf{z}}_{\text{new}},\tilde{\mathbf{z}}_{\text{old}}) - \beta F_{cos}(\tilde{\mathbf{z}}_{\text{new}}, \mathbf{z}),
%     \label{div}
% \end{equation}

where $F_{cos}$ refers to the cosine similarity loss. $d$ is a distance margin to avoid the augmented data totally overlapping with known data. $\alpha$ and $\beta$ are two hyper-parameters.

\noindent \textbf{Training the task model.} Given the known images $\mathbf{x}$, new and old augmented images $\tilde{\mathbf{x}}_{\text{old}}$ and $\tilde{\mathbf{x}}_{\text{new}}$. The overall loss function $\mathcal{L}_{\text{task}}$ for the task model is formulated as :
\begin{equation}
     \mathcal{L}_{\text{task}}=\mathcal{L}_{\text{cls}}(\mathbf{x}) + \mathcal{L}_{\text{metric}}(\mathbf{x},\tilde{\mathbf{x}}_{\text{old}}) + \mathcal{L}_{\text{metric}}(\mathbf{x},\tilde{\mathbf{x}}_{\text{new}}),
\end{equation}
where $\mathcal{L}_{\text{cls}}$ is a cross-entropy loss for known class classification, and $\mathcal{L}_{\text{metric}}$ is a triplet loss to distinguish the embedding of augmented data from known data, and simultaneously separating different known and augmented classes. $\mathcal{L}_{\text{metric}}$ is calculated on both new and old augmented data to avoid forgetting old open-set samples.
Specifically, different from existing works taking all simulated open-set samples as a single $K+1$ open class~\cite{zhou2021learning,neal2018open}, we assign different labels to augmented images from different known classes, as they carry diverse hybrid fingerprints. \eg, for input images of class $i$ and class $j$, we assign the augmented images by sending them into an augmentation model to different extended class labels $K+i$ and $K+j$. Then we sample triplets $\mathcal{T}$ from the merged images of input and augmented data. $\mathcal{L}_{\text{metric}}$ is calculated on triplet sets as follows:
\begin{equation}
    \mathcal{L}_{\text{metric}} = \sum_{\mathcal{T}_{z} \in \mathcal{T}} [\|x^{z}_{a} - x^{z}_{p}\|^{2}-\|x^{z}_{a}-x^z_{n}\|^{2}+ m]_{+} \label{metric},
\end{equation}
where $\mathcal{T}_{z}=(x_{a}^{z},x_{p}^{z},x_{n}^{z})$ is one triplet consisted of an anchor sample $x_{a}^{z}$, a positive sample $x_{p}^{z}$ and a negative sample $x_{n}^{z}$. $[\cdot]_{+}=\max(0,\cdot)$ denotes the hinge loss function. $m$ is the violate margin that requires the distance of negative pairs to be larger than the distance of positive pairs, by at least a margin $m$. By optimizing $\mathcal{L}_{\text{metric}}$, known and augmented data are distinguished, and different known and augmented classes are separated simultaneously.

 % $\mathcal{T}_{z}=(x_{a}^{z},x_{p}^{z},x_{n}^{z})$
% . Let $\bar{\mathbf{x}}=\mathbf{x}\cup\tilde{\mathbf{x}}$ be the merged images of input and augmented data, and $\mathcal{T}_{z}=(\bar{x}_{a}^{z},\bar{x}_{p}^{z},\bar{x}_{n}^{z})$ be one of the triplet set $\mathcal{T}$ sampled from $\bar{\mathbf{x}}$, 
% In a triplet set, $x_{a}$ is an anchor sample, $x_{p}$ is a positive sample with the same class as $x_{a}$, and $x_{n}$ is a negative sample of a different class from $x_{a}$. We sample triplet sets randomly from the merged images of input and augmented data. In merged images, the known images have classes from $1$ to $K$, and the augmented images are assigned to extended classes from $K+1$ to $2K$. By optimizing the triplet loss, the embedding of augmented data and known data are distinguished as they are in a negative relationship in the triplet set. Likewise, different known and augmented classes (2K classes in between) are separated as they are assigned different class labels. 

\noindent \textbf{Training and Testing Procedure.} The overall training progress is shown in Algorithm~\ref{alg::alg_pose}. In testing, the test image is fed into the feature extractor $F$ and classification head $H$, getting predicted confidence scores for each class after a $\textit{softmax}$ function. 
In practice, if the max confidence score is larger than a threshold $\theta$, the image is recognized as the known category corresponding to the index of the score. Otherwise, it is detected as unknown. We evaluate the 
overall closed/open discrimination performance by AUC and OSCR~\cite{dhamija2018reducing} calculated under diverse thresholds.


==> Sections/4_bak.tex <==
\section{Experiments}

\subsection{Experimental Details}


\noindent \textbf{Datasets.} We construct a benchmark for open-set model attribution. Table~\ref{tab:dataset_split1} shows single split of the benchmark (other 4 splits in the supplementary material), which contains 4 groups of images: seen real, seen fake, unseen real and unseen fake. Seen or unseen means whether images in the group is included in training set or not. Accordingly, we introduce these 4 groups as follows:
\begin{itemize}
	\item[$\bullet$] \textbf{Seen Real}: Subsets of 7 real dataset, which are CelebA~\cite{liu2015celeba}, Faces-HQ, ImageNet~\cite{deng2009imagenet}, Real Youtube images from Faceforensics~\cite{rossler2018faceforensics}, LSUN -Bedroom~\cite{yu2015lsun}, LSUN-Cat nd LSUN-Bus. Faces-HQ is the combination of two 1024 resolution face dataset, CelebA-HQ~\cite{karras2017progressive} and FFHQ~\cite{karras2019style}. 
% 	All seen real images are assigned `real' label.
	\item[$\bullet$] \textbf{Seen Fake}: Certain generative models trained on the seen real datasets above. For each real dataset, there are 2 models with different architectures trained on it. 
% 	Images generated by different models are assigned different labels.
	\item[$\bullet$]\textbf{Unseen Real}: Subsets of 2 real datasets that do not overlap with seen real datasets, which are CoCo~\cite{lin2014microsoft} and Summer Yosemite images~\cite{CycleGAN2017}.
	\item[$\bullet$] \textbf{Unseen Fake}: Unseen models share partly the same training settings with seen fake, but trained with different seed, architecture or dataset. The relationship between seen fake and unseen fake is shown in Table~\ref{tab:dataset_explain}. Unseen fake could be further divided into 3 categories: 
		\begin{itemize}
			\item[-] Unseen Seed: Unseen models having the same training dataset and architecture as certain seen models, but trained with different training seeds. 
			\item[-] Unseen Architecture: Unseen models trained on the same datasets as seen models, but with different architectures.
			\item[-] Unseen Dataset: Unseen models with the same architectures as certain seen models, but trained on different datasets.
		\end{itemize}
\end{itemize}
Figure~\ref{fig:dataset_explain2} shows the data split for the experiments. The training set contains seen real and seen fake. 
The testing set includes two parts: closed-set and open-set testing set. The closed-set contains images from known classes, including unseen real, seen real and seen fake. Note that unseen real is regarded as the `real' known class. Unseen fake all belong to unknown classes and form the open-set.

% \inputfigure{dataset_explain1}
\inputtable{dataset_explain}
\inputfigure{dataset_explain2}


\noindent \textbf{Evaluation.} 
We adopt accuracy to evaluate the attribution ability on the closed set. We use the area under ROC curve (AUROC) to evaluation the known/unknown discrimination performance. We also report Open Set Classification Rate (OSCR)~\cite{dhamija2018reducing} which measures the trade-off between accuracy and open-set detection rate as a threshold on the confidence of the predicted class is varied. 

\noindent \textbf{Implementation Details.} For the task models, we use a shallow 8-layer CNN network as the feature extractor. The output channel numbers for convolution layers are 64, 64, 128, 128, 256, 256, 512 and 512. Follow the feature extractor is a projection head and a classification head. We use a MLP with two hidden layers as the projection head. The projection head maps representations to the space where a metric loss is applied. We use a linear layer with dropout (p=0.2) as the classification head. For augment models, we use two-layer convolution networks, the output channel numbers are 32 and 3. We train a new augment model for every epoch. In training and inference, input images are firstly resized images to 128px. For optimization, we use Adam optimizer and the learning rate is multiplied by 0.9 for every 500 iterations. The initial learning rate is set to $10^{-4}$ for task models and $10^{-2}$ for augment models. The batch size is 8 $\times$ \#classes with a class balance strategy. More implementation details could be found in the supplementary material.

\inputtable{dataset_split1}

%The evaluation considers three aspects of performance: 
%1) We adopt accuracy to evaluate the attribution ability on the closed-set.
%2) We report AUROC to evaluation the known/unknown discrimination performance.
%3) To evaluate the ability of discovering new models, we report normalized mutual information (NMI) and purity following~\cite{}. 
%As NMI penalizes more on the cluster-level, and purity is not sensitive to the clustering number, we additionally report clustering accuracy to measure the realistic matching performance.

\noindent \textbf{Comparison Methods.} 
We compare against three groups of baselines: 1) GAN attribution methods, 2) GAN attribution and discovery method, and 3) open-set recognition methods. None of them are designed for open-set model attribution problem. The comparison methods and modifications to them are as follows:
\begin{itemize}
\item[$\bullet$] GAN attribution: PRNU~\cite{marra2019gans}, Yu \etal~\cite{yu2019attributing}, DCT-CNN~\cite{frank2020leveraging}, DNA-Det~\cite{yang2022aaai}, RepMix~\cite{bui2022repmix}. \cite{marra2019gans}, \cite{yu2019attributing} and \cite{frank2020leveraging} are under a closed-set model attribution setup. Although \cite{yang2022aaai} and \cite{bui2022repmix} are initially proposed for architecture attribution, we also evaluate them for model attribution. We train these five methods on the closed-set, and then obtain classification confidence scores on both the closed-set and open-set following the regular routine of OSR. The comparison results are shown in Table~\ref{tab:compare_attribution}.

\item[$\bullet$] GAN attribution and discovery: Girish \etal~\cite{girish2021towards} aims at the problem of open-world GAN attribution and discovery. Rather than focusing on recognizing knowns and distinguishing known/unknown simultaneously, ~\cite{girish2021towards} concentrates more on novel GAN discovery. We adapt our method into open world setting and compare with ~\cite{girish2021towards} in Table~\ref{tab:compare_openworld}.

\item[$\bullet$] Open-set recognition: four recent state-of-the-art generative methods for regular OSR problem, which are PROSER~\cite{zhou2021learning}, ARPL+CS~\cite{chen2021adversarial}, OpenGAN~\cite{kong2021opengan} and DIAS~\cite{moon2022difficulty}. For fair comparison, we use the same backbone for all these methods and our method. The comparison results are shown in Table~\ref{tab:compare_osr}.
\end{itemize}



\subsection{Evaluation of Open-set Model Attribution}
\inputtable{compare_attribution}
\inputtable{compare_openworld}

\noindent \textbf{Comparison with GAN attribution methods:} As shown in Table~\ref{tab:compare_attribution}, POSE outperforms existing fake image attribution methods with a large margin in terms of open-set recognition AUC and OSCR. Specifically, the AUC points on unseen seed, unseen architecture, unseen dataset and unseen all data are improved by 8.95, 2.44, 9.19, and 10.97, respectively. We can also observe that unseen seed data is the hardest open-set, unseen architecture is the next, and unseen dataset is the easiest, which is consistent with our intuition as unseen seed and unseen architecture data shares the same semantics as known classes, and unseen data even shares the same architecture. An exception case is that DNA-Det performs best on unseen architecture, but perform poorly on unseen dataset. This may because that unseen dataset classes have the same architectures as known classes and DNA-Det is proposed to extract architecture traces regardless of training dataset. 


\noindent \textbf{Comparison with GAN attribution and discovery method:} Girish \etal~\cite{girish2021towards} is proposed for open world GAN discovery and attribution. To compare with ~\cite{girish2021towards}, we train POSE on the labeled seen data and obtain features both seen and unseen data following the setup in \cite{girish2021towards}. Then features are clustered for 2 different values of $k$. $k=68$ corresponds to the true number of classes for all seen and unseen data. $k=49$ representss the number of clusters that \cite{girish2021towards} returns after 4 iterations. Average purity and Normalized Mutual Information (NMI) are calculated for evaluating the clustering performance. Results are shown in Table~\ref{tab:compare_openworld}. As seen, without iterative training on both seen and unseen data like \cite{girish2021towards}, POSE is able to outperform \cite{girish2021towards} in terms purity and get close NMI. These results validate the efficiency of POSE in reasoning about unseen GAN classes.

\noindent \textbf{Comparison with OSR methods:} We compare with OSR methods by simulating open-set in Table~\ref{tab:compare_osr}, which are PROSER~\cite{zhou2021learning}, ARPL+CS~\cite{chen2021adversarial}. We report the performance of a naive cross-entropy baseline without tricks proposed in them, which is the same with POSE w/o augmented models. We observe that PROSER~\cite{zhou2021learning} and ARPL+CS~\cite{chen2021adversarial} doesn't gain much improvements compared the baseline, which proves their generated open-set samples/features are not sub-optimal for open-set model attribution. 



\subsection{Ablation Study}

\inputtable{compare_osr}
\inputfigure{hist_compare}
\inputfigure{tsne_expansion}

\noindent \textbf{Validation of training with augment models:} As shown in Table~\ref{tab:compare_osr}, compared with a plain classifier training only on known samples (Base), applying augment models (Base+AM) in training not only improves classification accuracy of closed-set (from 90.67 to 93.41), but also largely improves closed/open set discrimination (from 73.13 to 80.31 in AUC on all unseen data). Specifically, the AUC points on unseen seed, unseen architecture and unseen dataset are improved by 5.11\%, 5.86\% and 9.53\% respectively. This indicates that simulating open space by augment models helps the feature extractor to extracts more distinguished features not only among close-set classes but also in between close/open-set.

\noindent \textbf{Validation of $\mathcal{L}_{\text{div}}$:} Figure~\ref{fig:tsne_expansion} gives an intuitive understanding of how $\mathcal{L}_{\text{div}}$ affects the open space expansion progress. As seen, with $\mathcal{L}_{\text{div}}$ added, the diversity of generated open space is largely increased. Further, we show in Figure~\ref{fig:tsne_expansion}(e) the pairwise similarity of open space expanded by each augment model with and without $\mathcal{L}_{\text{div}}$. We average pairwise similarity is [] without $\mathcal{L}_{\text{div}}$, while if $\mathcal{L}_{\text{div}}$ is employed, the similarity decreases to [], indicating again the ability of $\mathcal{L}_{\text{div}}$ to increase the divergence of augment models. The performances of POSE with and without $\mathcal{L}_{\text{div}}$ is presented in Table~\ref{tab:compare_osr}. We observe that with the help of $\mathcal{L}_{\text{div}}$, the AUC points on unseen seed, unseen architecture, unseen dataset and unseen all are improved by 4.24, 2.15, 2.84, and 2.40, respectively. The experimental results prove that the generated open space by employing $\mathcal{L}_{\text{div}}$ approaches closer to the real open space.


\noindent \textbf{The influence of augment model's architecture:} We vary the kernel size and number of layers of augment models to investigate the impact that different architectures of augment models have on close/open-set discrimination performance. Figure~\ref{fig:ablation_arch}(a) shows the open-set AUC \wrt kernels size of convolution layers, which indicates simulated open space by convolution layers of $3\times3$ kernel is the best for open model rejection. This is due to the fact that most GAN models use convolution layers with a $3\times3$ kernel size. In Figure~\ref{fig:ablation_arch}(b), we observe that the AUC reaches the summit when the number of augment model layer equals to 2 and keeps falling with K increasing. This is because only one layer is unable to produce rich open traces, and too many layers produce larger reconstruction residuals, which is too far away from known space.% to improve close/open discrimination. 
\inputfigure{ablation_arch}


% In Fig.~\ref{fig:hyper}(b), we observe that the open-set recognition AUC reaches the summit when $\epsilon=$ and drops when $\epsilon$ continuously increases, and the closed-set classification accuracy shows a similar curve. We take the open-set samples with a $\epsilon=$ reconstruction error as ``effective" samples. This phenomenon indicates that: 1) Too close or too distant simulated open samples are either ``effective", as the former would [] and the latter is too easy to reduce open-set risk. 2) Training with effective open-set samples would also aid the learning of known samples, as the feature extractor extracts more distinguished features not only in between close/open-set but also among close-set classes.  

\noindent \textbf{The influence of the number of augment models:} As a new augment model is trained for every epoch, we study the effect of the number of augmented models ($K$) by plotting the AUC under different training epochs in Figure~\ref{fig:ablation_K}.  We observe that the open-set recognition performance reaches the summit when $K = 17$ and remain stable with $K$ increasing. This is due to the fact more augmented models could hardly expand open space after certain number of augment models. Thus we select all POSE models at epoch 20 to produce the result. We also observe that the performance converges at early epochs without $\mathcal{L}_{\text{div}}$, indicating the necessity to increase the diversity of augment models in expanding open space. 

\inputfigure{ablation_K}



% We also compare with OpenGAN~\cite{kong2021opengan} in Fig.~\ref{fig:opengan}. We observe that the performance of OpenGAN vary largely with training epochs, even decreases up to [] between two neighboring epochs, epoch [] to epoch [] for instance. The performance of OpenGAN is largely related to eval/train mode and testing batch size. These phenomenons may be due to the fact that open features generated by OpenGAN tend to overlap with known class features, such that the discriminator is unstable in distinguishing close/open set. POSE is stable to all these factors, suggesting the efficiency of its generated samples.




==> Sections/4_experiment.tex <==
\section{Experiments}
 % There are four groups of data: Seen Real, Seen Fake, Unseen Real, and Unseen Fake\footnote{We also evaluation on newly arisen stable-diffusion~\cite{rombach2021highresolution} models in the later stage of this work, results are shown in the supplementary material.}, where Seen and Unseen mean whether images in this group are used for model attribution training or not. 
\subsection{Experimental Details}
\inputtable{dataset_1split}
\noindent \textbf{Datasets.} We construct a benchmark for open-set model attribution in Table~\ref{tab:dataset_1split}\footnote{Here we only present one way to split this benchmark. The other four splits of the benchmark are in the supplementary material.}. There are four groups of data: Seen Real, Seen Fake, Unseen Real, and Unseen Fake\footnote{We further include newly arisen stable-diffusion~\cite{rombach2021highresolution} models in the later stage of this work, results are shown in the supplementary material.}, where Seen and Unseen mean whether images in this group are used for model attribution training or not. Detailed descriptions are as follows:\\ %\hspace*{0.3cm} 
$\bullet$ \textbf{Seen Real}: Seven sets of real images: CelebA~\cite{liu2015celeba}, Faces-HQ (1024 resolution face images containing CelebA-HQ~\cite{karras2017progressive} and FFHQ~\cite{karras2019style}), ImageNet~\cite{deng2009imagenet}, Youtube (real Youtube images from Faceforensics++~\cite{roessler2019faceforensicspp}), Bedroom, Cat and Bus images of LSUN~\cite{yu2015lsun}. \\
$\bullet$ \textbf{Seen Fake}: Seen models trained on the seen real datasets in the same columns. Each real dataset trains two models of different architectures. \\ 
$\bullet$ \textbf{Unseen Real}: Images from two real datasets non-overlapping with the seen reals, including CoCo~\cite{lin2014microsoft} and Summer Yosemite images~\cite{CycleGAN2017}. \\
$\bullet$ \textbf{Unseen Fake}: Unseen models trained by partly the same settings with seen fake ones, but with different seeds, architectures, or training datasets. We control partly the same settings to consider the most challenging three scenarios. 
Please refer to Table~\ref{tab:dataset_explain} for the relationship between Seen and Unseen Fake.  Three categories of Unseen Fake are: \\
\hspace*{0.3cm} $-$ Unseen Seed: Unseen models of the same architecture and training data as certain seen fakes, but trained with different random seeds.\\
\hspace*{0.3cm} $-$ Unseen Architecture: Unseen models trained on the same datasets as seen fakes, but with different architectures. \\
\hspace*{0.3cm} $-$ Unseen Dataset: Unseen models of the same architecture as certain seen fakes, but trained on different datasets. 

In total, the benchmark contains 15 known classes including real and 14 seen models, and 53 unknown classes including 10 unseen seed models, 22 unseen architecture models and 21 unseen dataset models. To be realistic, as shown in Table~\ref{tab:train_test_split}, in the testing set, Unseen Real are also considered as closed-set samples as it should be taken as the same known `real' class as Seen Real, and Unseen Fake are taken as open-set classes. Compared with~\cite{girish2021towards}, our benchmark further considers two types of Unseen Fake (Unseen Seed and Unseen Dataset) and Unseen Real. 

\inputtable{alg_pose}
\inputtable{dataset_explain}
\noindent \textbf{Evaluation.} The performance is evaluated in two aspects: accurately classifying the known models, and distinguishing known and unknown models correctly, which are measured by accuracy and the area under ROC curve (AUC) respectively. We also report Open Set Classification Rate (OSCR) measuring the trade-off between the two aspects.

\noindent \textbf{Implementation details.} 
For the task model, the feature extractor includes a discrete cosine transform (DCT) transformation layer and a simple convolution network same as DNA-Det~\cite{yang2022aaai}. The reason for the DCT layer is that we find the distinctions of fingerprints in the frequency domain are more obvious than in the pixel domain. With the plain task model with by a cross-entropy loss, the closed-set accuracies are 90.67\% and 83.53\% for DCT and RGB input, while the AUCs on all unseen data are similar (73.78\% and 74.26\%). The classification head is an MLP network with two linear layers. The augmentation models have two convolution layers, whose weight shapes are $3\times32\times3\times3$ and $32\times3\times3\times3$, respectively. For optimization, we use the Adam optimizer with a step scheduler. The initial learning rate is set to $10^{-4}$ for task models and $10^{-2}$ for augmentation models. The hyper-parameter $\lambda$ in $\mathcal{L}_{\text{spectral}}$ is set to $10^{-4}$. For the hyper-parameters in $\mathcal{L}_{\text{div}}$, we empirically set $\alpha=10^{-4}$, $\beta=10^{-2}$, and $d=0.95$. The violate margin $m$ in $\mathcal{L}_{\text{metric}}$ is set to 0.3. Input images are all resized to 128px before sending into the network. 

\noindent \textbf{Compared methods.} 
We compare against three groups of baselines: 1) GAN attribution, 2) GAN discovery and 3) open-set recognition methods. Most of them are not designed for the open-set model attribution problem. Compared methods and modifications to them are as follows: \\ %\hspace*{0.3cm} 
$\bullet$ \textbf{GAN attribution}: PRNU~\cite{marra2019gans}, Yu \etal~\cite{yu2019attributing}, DCT-CNN~\cite{frank2020leveraging}, DNA-Det~\cite{yang2022aaai}, and RepMix~\cite{bui2022repmix}. We train them on the closed-set, and then obtain classification confidence scores on both the closed-set and open-set following the regular routine of OSR. Comparison results are in Table~\ref{tab:compare_attribution}. \\
$\bullet$ \textbf{GAN discovery}: Girish \etal~\cite{girish2021towards} focus on discovering newly arisen unseen GANs. To compare with this work, we first train on the closed-set, and extract features for both the closed-set and open-set following the setup in \cite{girish2021towards}, which are clustered by K-Means with the true cluster number and predicted cluster number by \cite{girish2021towards}. Results are in Table~\ref{tab:compare_openworld}.\\
$\bullet$ \textbf{Open-set recognition}: The classical discriminative OSR method OpenMax~\cite{bendale2016towards} and three state-of-the-art generative OSR methods: PROSER~\cite{zhou2021learning}, ARPL+CS~\cite{chen2021adversarial}, and DIAS~\cite{moon2022difficulty}. Comparison results are in Table~\ref{tab:compare_osr}.

\inputtable{train_test_split}
\inputtable{compare_attribution}

\subsection{Evaluation of Open-Set Model Attribution}

\noindent \textbf{Comparison with GAN attribution methods.} As shown in Table~\ref{tab:compare_attribution}, POSE outperforms existing fake image attribution methods by a large margin in terms of AUC and OSCR. Specifically, the AUC points on unseen architecture, unseen dataset, and unseen all data are improved by 3.24\%, 9.45\%, and 11.02\%, respectively, indicating the superiority of POSE in open-set discrimination. PRNU~\cite{marra2019gans} achieves slightly higher AUC on seen seed, which may be because filters to extract PRNU noise are rather sensitive to differences in traces brought by model weights. We can also observe that unseen seed is the hardest open-set, unseen architecture the second, and unseen dataset is the easiest, which is consistent with our intuition as unseen seed and unseen architecture data only differ from seen data in visually imperceptible traces, and unseen seed data even shares the same model architecture. An exception case is DNA-Det~\cite{yang2022aaai}, which performs well on unseen architecture, but poorly on unseen dataset. This is due to the fact that DNA-Det is designed to extract architecture traces regardless of the training dataset, yet data in unseen dataset share the same model architectures as seen data.
\inputtable{compare_openworld}
% \inputfigure{hist_compare}
\inputfigure{hist_tsne}

\noindent \textbf{Comparison with the GAN discovery method.} To compare with Girish \etal~\cite{girish2021towards} in discovering unseen models, we train POSE on seen data and obtain features for both the seen and unseen data, which are then clustered for two different values of cluster number $k$. $k=68$ corresponds to the true number of classes for seen and unseen data. $k=49$ represents the number of clusters that \cite{girish2021towards} returns after four iterations. Average purity, Normalized Mutual Information (NMI), and Adjusted Rand Index (ARI) are calculated to evaluate the clustering performance. Results are shown in Table~\ref{tab:compare_openworld}. As seen, without iterative training on both seen and unseen data like \cite{girish2021towards}, POSE is able to outperform in terms of purity and ARI, and get close NMI, which validates the efficiency of POSE in reasoning about unseen GAN classes. \\
\noindent \textbf{Comparison with OSR methods.} We take 
optimizing the plain task models by a cross-entropy loss as a Base method, and compare with OpenMax~\cite{bendale2016towards}, PROSER~\cite{zhou2021learning}, ARPL+CS~\cite{chen2021adversarial}, and DIAS~\cite{moon2022difficulty} by employing their proposed techniques and simulated open-set samples to augment the Base classifier. As shown in Table~\ref{tab:compare_osr}, applying augmentation models (Base+AM) is superior to other OSR methods, and involving $\mathcal{L}_{\text{div}}$ (Base+AM+$\mathcal{L}_{\text{div}}$) gains further improvement. These results prove that the simulated open space by POSE is more suitable for OSMA than off-the-shelf OSR methods. 
\subsection{Ablation Study}
\label{sec:ablation}
\inputtable{compare_osr}
\inputfigure{tsne_expansion}

\noindent \textbf{Validation of training with augmentation models.} As shown in Table~\ref{tab:compare_osr}, compared with the Base method, applying augmentation models (Base+AM) not only improves closed-set classification accuracy (from 90.68\% to 93.41\%) but also helps open-set discrimination (from 73.78\% to 80.31\% in AUC on unseen all data). This indicates simulating open space by augmentation models helps more compact feature extraction not only among close-set classes but also in between close/open-set. Meanwhile, observing the feature space visualization cases in Figure~\ref{fig:hist_tsne}(top), the augmented data simulates a rich open space enclosing the known data points, resulting in a clear better close/open discrimination.  Better open-set discrimination is also reflected in the prediction confidence scores in Figure~\ref{fig:hist_tsne}(below), again justifying the effect of augmentation models.

\noindent \textbf{Validation of $\mathcal{L}_{\text{div}}$.} Figure~\ref{fig:tsne_expansion}(a-d) give an intuitive understanding of how $\mathcal{L}_{\text{div}}$ influences the open space expansion progress. As seen, with $\mathcal{L}_{\text{div}}$ added, the diversity of open space simulated by different augmentation models is largely increased, which is also indicated in the decreased pairwise similarity in Figure~\ref{fig:tsne_expansion}(e). Further, with the help of $\mathcal{L}_{\text{div}}$, the AUC points on unseen seed, architecture, dataset and unseen all data increase by 1.98\%, 1.96\%, 3.20\%, and 2.45\%. These results prove that employing $\mathcal{L}_{\text{div}}$ increases the diversity of simulated open space and reduces the open space risk better.

\inputfigure{ablation_arch}
\noindent \textbf{Validation of the architecture of augmentation models.} 
We investigate the impact that the augmentation model's architecture has on open-set discrimination performance from three aspects: 1) Upsampling layer. As discussed in Section~\ref{sec:m0}, including upsampling in the augmentation model would heavily influence high frequencies and tend to produce trivial open-set samples. We empirically include upsampling layer in the augmentation model (Down+Conv+Up+Conv), resulting in much lower performance than two pure convolution layers (Conv+Conv) shown in Figure~\ref{fig:ablation_arch}(a), which verifies our former assumption. 2) Layer number. In Figure~\ref{fig:ablation_arch}(b), the AUC reaches the summit when the convolution layer number equals 2 and decreases with more layers. This may be due to that a single layer is hard to simulate large open space, while more layers lead to larger reconstruction residuals and produce easier open-set samples far from known space. 3) Kernel size. Figure~\ref{fig:ablation_arch}(c) shows the AUC \wrt kernel size of convolution layers, indicating a $3\times3$ kernel size is the best. This could be because most generative models use a $3\times3$ kernel size. 

\noindent \textbf{Progressive vs. joint training.} It is computation-expensive to jointly train a large number of augmentation models one-off and constrain the diversity among them. We compare the OSR performance of progressive and joint training with 9 augmentation models (the maximum number of augmentation models could be trained jointly on a 32G V100 GPU) on one split. At the 9th epoch with the same number of augmentation models involved, AUCs on unseen all data under progressive and joint training are 80.17\% and 79.42\%, while the latter takes five times longer to train than the former, which indicates progressive training provides an effective way to expand the open space.

\inputfigure{ablation_K}
\noindent \textbf{Influence of the number of augmentation models.} We study the effect of the number of augmentation models ($N$) in improving open-set recognition performance by plotting the AUCs and accuracies under different training epochs on one split in Figure~\ref{fig:ablation_K}. We can observe that the performance converges at early epochs without $\mathcal{L}_{\text{div}}$, while the AUC of POSE increases continually until about 19 epochs, indicating the necessity to increase the diversity of simulated open space. 


% We also compare with OpenGAN~\cite{kong2021opengan} in Fig.~\ref{fig:opengan}. We observe that the performance of OpenGAN vary largely with training epochs, even decreases up to [] between two neighboring epochs, epoch [] to epoch [] for instance. The performance of OpenGAN is largely related to eval/train mode and testing batch size. These phenomenons may be due to the fact that open features generated by OpenGAN tend to overlap with known class features, such that the discriminator is unstable in distinguishing close/open set. POSE is stable to all these factors, suggesting the efficiency of its generated samples.




==> Sections/5_conclusion.tex <==

% which promotes the application of model attribution  unseen real images and 
\section{Conclusions and Future Work}
This paper tackles an important problem in applying model attribution to the real world, the open-set model attribution problem, to attribute images to known source models and identify those from unknown ones. We propose a novel progressive open space expansion solution for this problem, whose core idea is to simulate the potential open space of unknown models by involving augmentation models progressively. We consider three challenging types of unknown models to construct a benchmark simulating the real world attribution scenario. The superior experimental results indicate that it is promising to model the boundary of known models by artificially constructed models. In the future, it is fruitful to study how fingerprints are dominated by network components and simulate them by artificial tiny networks. This may result in better fingerprint space representation for more generic model attribution.



% limits
% 1. Robustness: fine-tune, post-processing
% 2. Unseen seed is challenging
% 3. the simulated open space is still limited

% Future work
% 1.  It's fruitful is study how fingerprints are dominated by network components, architecture and weights. Whether it's possible to utilize tiny networks to pretrain a ssl network. Face recogntion.
% 2. 


==> Sections/6_ack.tex <==
\section{Acknowledgements}
The research work is supported by the China Postdoctoral Science Foundation (2022TQ0344), the Project of Chinese Academy of Sciences (E141020), the National Natural Science Foundation of China (62203425), and the Zhejiang Provincial Key Research and Development Program of China (No.2021C01164).

==> Sections/7_sup.tex <==
% \begin{overview}
The supplementary material is organized as follows:
\begin{itemize}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
\item 
Section~\ref{sec:sup_s2} provides the open-set discrimination result on images generated by a stable-diffusion model.
\item 
Section~\ref{sec:sup_s3} gives an analysis on two situations for open-set model attribution: unseen seed model and fine-tuned model.
\item
Section~\ref{sec:sup_s1} gives robustness analysis against common image perturbations. 
\item 
Section~\ref{sec:sup_s4} shows the full five splits of the OSMA benchmark. 
\item
Section~\ref{sec:sup_s5} visualizes randomly selected samples from the OSMA benchmark.
\end{itemize}
% \end{overview}

\section{Evaluation on Diffusion Model}
\label{sec:sup_s2}
We evaluate samples generated by the newly arisen stable-diffusion model~\cite{rombach2021highresolution}. We use CoCo~\cite{lin2014microsoft} captions to generate 1k stable-diffusion samples and test POSE's open-set discrimination performance on these samples. Randomly selected samples are shown in Figure~\ref{fig:diffusion_samples}. As shown in Figure~\ref{fig:diffusion_hist}, the AUC point between closed-set and unseen stable-diffusion samples is 92.40, indicating that POSE is able to capture the difference in traces of known models and stable-diffusion model, and recognize stable diffusion samples as from a new model. 
\inputfigure{diffusion_hist}

\section{Unseen Seed and Finetuned Model}
\label{sec:sup_s3}
\inputfigure{ft_seed_hist}
For open-set model attribution, there exist two situations near the known space boundary, \textit{i.e.}, models trained with only seed different, and models fine-tuned from the known models. To analyze how POSE reacts in the two situations, we train a 2-way POSE classifier on \{celeba, ProGAN\_celeba\_seed0\}, and test the classifier on seven unseen models including ProGAN\_celeba\_seed1, and six models finetuned from ProGAN\_celeba\_seed0 on the celeba dataset. We plot in Figure~\ref{fig:ft_seed_hist} the confidence histograms for these models and calculate the weight distance between seen ProGAN\_celeba\_seed0 model and seven unseen models. Specifically, the weight distance between two models is calculated as follows:
\begin{equation}
D(W_{1}, W_{2}) = \frac{1}{N}\sum_{i=1}^{N}\frac{\|W_{2,i}-W_{1,i}\|}{\|W_{1,i}\|},
\end{equation}
where $W_{1}$ and $W_{2}$ are weights of two models with the same architecture. $N$ is the number of layers that are equipped with learnable weights. 

As shown in Figure~\ref{fig:ft_seed_hist}, the POSE classifier is able to separate samples generated by an unseen seed model (ProGAN\_celeba\_seed1) from seen ProGAN\_celeba\_seed0 model. With the finetune step increases (from 200 to 5000), the weight distance between the finetuned model and the original ProGAN\_celeba\_seed0 model increases followingly (from 0.001 to 0.019). When the weight distance reaches 0.019, POSE achieves a clear separation between the finetuned model and the original model. These results indicate that POSE is sensitive to trace changes brought by model weight changes, and is suitable for scenarios requiring strict attribution.


\section{Robustness Analysis}
\label{sec:sup_s1}

\inputfigure{diffusion_samples}
\inputfigure{robustness}

Generated images may undergo post-processings in real-world scenarios. We evaluate the robustness of POSE against five common image perturbations, which are Blurring with Gaussian, JPEG compression, Lighting, additive Gaussian noise, crop, and resize. We evaluate the original version and immunized version of POSE. The original version indicates the perturbation is not included in model training, and the immunized version indicates that the perturbation is included as a kind of data augmentation in model training. We plot the OSCR results w.r.t the strength of each perturbation in Figure~\ref{fig:robustness}. As seen, without immunization, image perturbations would largely influence the model attribution performance. Nevertheless, with image perturbations included as data augmentation operations in model training, the performance drop is largely relieved. Specifically, the immunized version is rather robust to Lighting, Noise, and Crop perturbations. For JPEG compression quality $\sim$ [80, 100], and blur kernel size $\sim$ [0, 3], the performance drop could maintain within a 10\% range.


\section{Full Dataset Splits}
\label{sec:sup_s4}

\inputtable{dataset_split1}
\inputtable{dataset_split2}
\inputtable{dataset_split3}
\inputtable{dataset_split4}
\inputtable{dataset_split5}

We provide the full five splits of the OSMA benchmark in Table~\ref{tab:dataset_split1}, Table~\ref{tab:dataset_split2}, Table~\ref{tab:dataset_split3}, Table~\ref{tab:dataset_split4}, and Table~\ref{tab:dataset_split5}, in which Table~\ref{tab:dataset_split1} is the same as Table 1 in the main text.

\section{Visualization of Dataset Samples}
\label{sec:sup_s5}

\inputfigure{samples}
We provide randomly selected samples in the benchmark for models trained on CelebA, Face-HQ, ImageNet, Youtube, LSUN-Bedroom, LSUN-Cat, and LSUN-Bus, which are shown in Figure~\ref{fig:samples}.









==> Tables/alg_pose.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}} 
\renewcommand{\algorithmicensure}{\textbf{Output:}} 
\begin{algorithm}[t]
  \caption{Progressive Open-Space Expansion (POSE)}
  \label{alg::alg_pose}
  \begin{algorithmic}[1]
    \Require
      Known class images $\mathbf{x}$; 
      Number of epochs $N$
    \Ensure
      Learned task model $M$; Learned augmentation models $\{A_{i}\}_{i=0}^{N-1}$
    \For{$i = 0, \dots, N$} 
        \State Generate augmented images $\tilde{\mathbf{x}}_{\text{new}}$ with $A_{i}(\mathbf{x})$
        \If{$i=0$}
            %\State Generate augment image $\tilde{\mathbf{x}}_{\text{new}}$ using $A_{0}$
            \State Train $A_{0}$ by $\mathcal{L_{\text{recons}}}(\mathbf{x},\tilde{\mathbf{x}}_{\text{new}})$
            % \State Train task model $M$ using $\mathcal{L_{\text{task}}}$
            % \State Train task model $M$ using $\mathcal{L}_{\text{task}}(\mathbf{x},\tilde{\mathbf{x}}_{\text{new}})$
        \Else
            \State Randomly select $j$ from $0$ to $i-1$
            \State Generate augmented image $\tilde{\mathbf{x}}_{\text{old}}$ with $A_{j}(\mathbf{x})$
            %\State Randomly select a previously trained augmentation model, and generate augmented images $\tilde{\mathbf{x}}_{\text{old}}$
            %\State Generate augmented images $\tilde{\mathbf{x}}_{\text{new}}$ using $A_{i}$
            \State Train $A_{i}$ by $\mathcal{L_{\text{recons}}}(\mathbf{x},\tilde{\mathbf{x}}_{\text{new}})$ and $\mathcal{L_{\text{div}}}(\tilde{\mathbf{x}}_{\text{old}},\tilde{\mathbf{x}}_{\text{new}})$
            % \State Train task model $M$ using $\mathcal{L_{\text{task}}}$
            % \State Train task model $M$ using $\mathcal{L}_{\text{task}}(\mathbf{x},\tilde{\mathbf{x}}_{\text{old}},\tilde{\mathbf{x}}_{\text{new}})$
        \EndIf
        %\State Generate augmented images $\tilde{\mathbf{x}}_{\text{new}}$ using $A_{i}$
        \State Train the task model $M$ using $\mathcal{L}_{\text{task}}$
    \EndFor
  \end{algorithmic}
\end{algorithm}

% \noindent \textbf{Testing.} 


==> Tables/compare_attribution.tex <==
% \begin{table*}[t!]
% \setlength{\abovecaptionskip}{2mm}
% \caption{Comparison with existing GAN attribution methods. Results are averaged among five splits of the benchmark.}
% \centering
% \begin{tabular}{llccccccccccccc}
% \toprule
% \multirow{2}{*}{Method} & \multirow{2}{*}{Publish} & Closed-Set & & \multicolumn{2}{c}{Unseen Seed} & & \multicolumn{2}{c}{Unseen Architecture} & & \multicolumn{2}{c}{Unseen Dataset} & & \multicolumn{2}{c}{Unseen All} \\  
% % \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} \cmidrule{10-11}  \cmidrule{13-14} 
% \cmidrule{3-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}  \cmidrule{14-15} 
%  & & Accuracy & & AUC  & OSCR  & &  AUC  & OSCR & & AUC  & OSCR & &  AUC  & OSCR \\
% \midrule
% PRNU et al.~\cite{marra2019gans} & MIPR2019 & \\
% Yu~\etal~\cite{yu2019attributing} & ICCV2019 & 85.71 &&	53.14 &	50.99 &&	69.04 &	64.17 &&	78.79 &	72.20 &&	69.90 &	64.86  \\
% DCT-CNN~\cite{frank2020leveraging} & ICML2020 & 86.16 &&	55.46 &	52.68 &&	72.56 &	67.43 &&	72.87 &	67.57 &&	69.46 &	64.70  \\
% DNA-Det~\cite{yang2022aaai}  & AAAI2022 & 93.56 &&	61.46 &	59.34 &&	80.93 &	76.45 &&	66.14 &	63.27 &&	71.40 &	68.00 \\
% RepMix ~\cite{bui2022repmix} & ECCV2022 & 93.69 &&	54.70 &	53.26 &&	72.86 &	70.49 &&	78.69 &	76.02 &&	71.74 &	69.43 \\
% \midrule
% \textbf{POSE} & & \textbf{94.49}  &&	\textbf{70.41} &	\textbf{69.08} &&	\textbf{83.37} &	\textbf{80.67} &&	\textbf{87.88} &	\textbf{85.03} &&	\textbf{82.71} &	\textbf{80.21} \\
% %   &  \increase{0.80} &&	 \increase{8.95}  &	\increase{69.08} &&	\increase{83.37} &	\increase{80.67} &&	\increase{87.88} &	\increase{85.03} &&	\increase{82.71} &	\increase{80.21} \\
% \bottomrule
% \end{tabular}
% \label{tab:compare_attribution}
% \vspace{-5mm}
% \end{table*}



\begin{table*}[t!]
\setlength{\abovecaptionskip}{2mm}
\caption{Comparison with existing GAN attribution methods. Results are averaged among five splits of the benchmark.}
\centering
\begin{tabular}{lccccccccccccc}
\toprule
\multirow{2}{*}{Method} & Closed-Set & & \multicolumn{2}{c}{Unseen Seed} & & \multicolumn{2}{c}{Unseen Architecture} & & \multicolumn{2}{c}{Unseen Dataset} & & \multicolumn{2}{c}{Unseen All} \\  
\cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} \cmidrule{10-11}  \cmidrule{13-14}  
 & Accuracy & & AUC  & OSCR  & &  AUC  & OSCR & & AUC  & OSCR & &  AUC  & OSCR \\
\midrule
PRNU~\cite{marra2019gans} & 55.27 && \textbf{69.20} &	49.16 &&	70.02 &	49.49&& 	67.68 &	48.57 &&	68.94 &	49.06 \\
Yu~\etal~\cite{yu2019attributing} & 85.71 &&	53.14 &	50.99 &&	69.04 &	64.17 &&	\underline{78.79} &	72.20 &&	69.90 &	64.86  \\
DCT-CNN~\cite{frank2020leveraging} & 86.16 &&	55.46 &	52.68 &&	72.56 &	67.43 &&	72.87 &	67.57 &&	69.46 &	64.70  \\
DNA-Det~\cite{yang2022aaai}  & 93.56 &&	61.46 &	\underline{59.34} &&	\underline{80.93} &	\underline{76.45} &&	66.14 &	63.27 &&	71.40 &	68.00 \\
RepMix~\cite{bui2022repmix} & \underline{93.69} &&	54.70 &	53.26 &&	72.86 &	70.49 &&	78.69 &	\underline{76.02} &&	\underline{71.74} &	\underline{69.43} \\
\midrule
% \textbf{POSE} & \textbf{94.49}  &&	\textbf{70.41} &	\textbf{69.08} &&	\textbf{83.37} &	\textbf{80.67} &&	\textbf{87.88} &	\textbf{85.03} &&	\textbf{82.71} &	\textbf{80.21} \\
 % \textbf{POSE} & \textbf{94.72} && \textbf{69.76} 	& \textbf{68.41} 	&& \textbf{83.98} 	&\textbf{81.17} &&	\textbf{88.13} &	\textbf{85.18} &&	\textbf{82.94} &	\textbf{80.36} \\
\textbf{POSE} & \textbf{94.81} &&	\underline{68.15} &	\textbf{67.25} &&	\textbf{84.17} &	\textbf{81.62} &&	\textbf{88.24} &	\textbf{85.64} &&	\textbf{82.76} &	\textbf{80.50}  \\ %new model with margin
\bottomrule
\end{tabular}
\label{tab:compare_attribution}
\vspace{-5mm}
\end{table*}


==> Tables/compare_openworld.tex <==
  
\begin{table}[t]
\setlength\tabcolsep{2.0pt}
\setlength{\abovecaptionskip}{2mm}
\caption{Comparision with Girish~\etal~\cite{girish2021towards} for GAN discovery.}
\centering
\begin{tabular}{lcccccccccccc}
\toprule
Method & Avg. Purity & NMI & ARI \\
\midrule
Girish~\etal~\cite{girish2021towards} (k=49) & 32.89 & 61.89 & 21.05 \\
% POSE (k=49) & 40.94 & 62.55 & 29.15 \\ old model with margin
% POSE (k=49) & 38.30 & 61.30 & \textbf{26.54} \\ %new model without margin
\textbf{POSE} (k=49) & 39.16 & \textbf{61.91} & \textbf{27.48} \\ %new model with margin
% POSE (k=68) & 43.28 & 61.57 & 28.30 \\
\textbf{POSE} (k=68) & \textbf{41.04} & 60.59 & 26.39 \\
% POSE* (k=68) &   \\
\bottomrule
\end{tabular}
\label{tab:compare_openworld}
\vspace{-3mm}
\end{table}
  
 


==> Tables/compare_osr.tex <==
\begin{table*}[t]
% \setlength\tabcolsep{1pt}
% \begin{tabular}{
% p{3.5cm}
% p{2cm}<{\centering}p{0.1cm}<{\centering}
% p{1.3cm}<{\centering}
% p{1.3cm}<{\centering}p{0.1cm}<{\centering}
% p{1.3cm}<{\centering}
% p{1.3cm}<{\centering}p{0.1cm}<{\centering}
% p{1.3cm}<{\centering}
% p{1.3cm}<{\centering}p{0.1cm}<{\centering}
% p{1.3cm}<{\centering}
% p{1.3cm}<{\centering}
% }
% The best and second-best results are boldfaced and underlined.
\setlength{\abovecaptionskip}{2mm}
\caption{Comparison with existing OSR methods and ablation experiments. Results are averaged among five splits of the benchmark. }
\centering
\scalebox{0.95}{
\begin{tabular}{lccccccccccccc}
\toprule
\multirow{2}{*}{Method} & Closed-Set & & \multicolumn{2}{c}{Unseen Seed} & & \multicolumn{2}{c}{Unseen Architecture} & & \multicolumn{2}{c}{Unseen Dataset} & & \multicolumn{2}{c}{Unseen All} \\  
\cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8} \cmidrule{10-11}  \cmidrule{13-14} 
 & Accuracy & & AUC  & OSCR  & &  AUC  & OSCR & & AUC  & OSCR & &  AUC  & OSCR \\
\midrule
% Base & 90.67 &&	61.06 &	59.82 &&	76.35 &	73.25 &&	75.51 &	72.58 &&	73.13 &	70.45 \\
% Base+OpenMax~\cite{bendale2016towards}\ & 91.11&& 	63.27 &	\underline{61.60} &&	76.40 &	73.29 &&	75.33 &	72.32 &&	73.50 &	70.70 \\
% Base+PROSER~\cite{zhou2021learning} &   92.02 && \underline{65.00} & - && \underline{79.67} & - && 80.81 & - && 77.31& -\\
% % Base+ARPL+CS~\cite{chen2021adversarial} &  91.61 &&	65.79 &	64.31 && 78.27 & 75.24 && 76.88 &	74.20 &&	75.36 &	72.76 	\\
% Base+ARPL+CS~\cite{chen2021adversarial} &91.77 &&	54.94& 	54.17&& 	79.09& 	75.97 &&	80.48& 	77.52&& 	75.08& 	72.47 \\ 
% Base+DIAS~\cite{moon2022difficulty} &  \underline{92.77} &&	62.15 &	61.02 &&	79.34 &	\underline{76.49} &&	\underline{84.14} &	\underline{81.13} &&	\underline{78.00} &	\underline{75.41} \\
% GCD~\cite{vaze2022openset} & \\
% Base & 90.67 &&	61.06 &	59.82 &&	76.35 &	73.25 &&	75.51 &	72.58 &&	73.13 &	70.45 \\
Base & 90.68 &&	62.02 &	60.58 	&&76.03 &	72.92 &&	77.01 &	73.88 &&	73.78 &	70.97 \\
Base+OpenMax~\cite{bendale2016towards}\ & 91.11&& 	63.27 &	61.60 &&	76.40 &	73.29 &&	75.33 &	72.32 &&	73.50 &	70.70 \\
% Base+PROSER~\cite{zhou2021learning} &   92.02 && 65.00 & - && 79.60 & - && 80.81 & - && 77.31& -\\
Base+PROSER~\cite{zhou2021learning} & 92.12	&& 63.32&	62.19&&	79.55&	76.57&&	81.43&	78.64&&	77.22&	74.66 \\
Base+ARPL+CS~\cite{chen2021adversarial} &91.77 &&	54.94& 	54.17&& 	79.09& 	75.97 &&	80.48& 	77.52&& 	75.08& 	72.47 \\ 
Base+DIAS~\cite{moon2022difficulty} &  92.77 &&	62.15 &	61.02 &&	79.34 &	76.49  &&84.14 &	81.13 && 78.00 &	75.41 \\
\midrule
Base+AM & \underline{93.41} &&	\underline{66.17} &	\underline{65.04} &&	\underline{82.21} &	\underline{79.42} &&	\underline{85.04} &	\underline{82.20} &&	\underline{80.31} &	\underline{77.80} \\ 
% Base+AM+$\mathcal{L}_{\text{div}}$  & \textbf{94.49} &&	\textbf{70.41} &	\textbf{69.08} &&	\textbf{83.37} &	\textbf{80.67} &&	\textbf{87.88} &	\textbf{85.03} &&	\textbf{82.71} &	\textbf{80.21} \\
% Base+AM+$\mathcal{L}_{\text{div}}$   & \textbf{94.72} && \textbf{69.76} 	& \textbf{68.41} 	&& \textbf{83.98} 	&\textbf{81.17} &&	\textbf{88.13} &	\textbf{85.18} &&	\textbf{82.94} &	\textbf{80.36} \\
Base+AM+$\mathcal{L}_{\text{div}}$(\textbf{POSE})  & \textbf{94.81} &&	\textbf{68.15} &	\textbf{67.25} &&	\textbf{84.17} &	\textbf{81.62} &&	\textbf{88.24} &	\textbf{85.64} &&	\textbf{82.76} &	\textbf{80.50}  \\
\bottomrule
\end{tabular}}
\label{tab:compare_osr}
\vspace{-5mm}
\end{table*}


==> Tables/dataset.tex <==
\begin{table*}
\small
\caption{List of dataset used in our experiments, including 4 groups: seen real, seen models, unseen real and unseen models.} 
\setlength\tabcolsep{0.5pt}
\begin{center}
\begin{tabular}{llllll}
\toprule
&  & \multicolumn{3}{c}{Unseen Models}  & \\
\cmidrule{3-5} 
Seen Real &  Seen Models  & Unseen Seed &  Unseen Arch. & Unseen Dataset & Unseen Real \\
\midrule
CelebA & ProGAN\_s0, StarGAN &  ProGANs\_s1-ProGAN\_s5 & AttGAN, SNGAN, MMDGAN CramerGAN &  GauGAN\_CoCo & CoCo \\
Faces-HQ & ProGAN, StyleGAN &   - & StyleGAN2, ResNet19 & CRN\_GTA & GTA \\
ImageNet & BigGAN, S3GAN &  - & SNGAN, ContraGAN, SAGAN & CycleGAN\_Summer & Summer \\
LSUN & ProGAN\_s0, MMDGAN &  ProGANs\_s1-ProGAN\_s5 & SNGAN, CramerGAN & CycleGAN\_Horse & Horse\\
Youtube & FSGAN, Faceshifter & - & Wav2Lip, FaceSwap \\
\bottomrule
\end{tabular}
\end{center}
\label{tab:dataset}
\end{table*}

==> Tables/dataset_1split.tex <==

% \yty{more explanations,seen, unseen, known, unknown, closed-set, open-set, easy to confuse reviewers,open-set include both known classes and unknown classes, or unknown classes only?}
\begin{table*}[t]
\setlength\tabcolsep{1.8pt}
\setlength{\abovecaptionskip}{2mm}
\caption{One split of the OSMA benchmark, including four groups: Seen Real, Seen Fake, Unseen Real, and Unseen Fake. Models in each column of Seen Fake, Unseen Seed, and Unseen Architecture are trained on the corresponding Seen Real dataset in the same column. Unseen Dataset include a total of 21 ProGAN, StyleGAN, and StyleGAN models trained on 7 datasets non-overlapping with Seen Real.}
\centering
\scalebox{0.83}{
\begin{tabular}{lllllllll}
\toprule[1.5pt]
% seen real
\multicolumn{2}{c}{\textbf{Seen Real}} & CelebA & Face-HQ & ImageNet & Youtube & LSUN-Bedroom & LSUN-Cat & LSUN-Bus \\
% seen fake
\midrule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Seen Fake}}} &
\multirow{2}{\celllargewidth}{StarGAN\cite{choi2018stargan},\\ProGAN\_seed0\cite{karras2017progressive}} & \multirow{2}{\celllargewidth}{StyleGAN3-r\cite{karras2021alias}, \\StyleGAN3-t} & \multirow{2}{\cellbigwidth}{SAGAN\cite{zhang2019self},\\SNGAN} & 
\multirow{2}{\cellbigwidth}{FSGAN\cite{nirkin2019fsgan}, \\FaceSwap\cite{faceswap}} & 
\multirow{2}{\cellmidwidth}{ProGAN\_seed0, \\MMDGAN} & 
\multirow{2}{\cellmidwidth}{StyleGAN, \\StyleGAN3} & 
\multirow{2}{\cellmidwidth}{ProGAN, \\StyleGAN} \\ \\
% unseen fake
% % unseen seed
\midrule
\multirow{8}{\cellsmallwidth}{\textbf{Unseen \\Fake}} & \multirow{2}{\cellsmallwidth}{\textbf{Unseen \\Seed}} &
\multirow{2}{\celllargewidth}{ProGAN\\(seed1,2,3,4,5)} & 
\multirow{2}{\celllargewidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{ProGAN\\(seed1,2,3,4,5)} & 
\multirow{2}{\cellmidwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{\centering -} \\\\
% % unseen arch
\cmidrule{2-9}
& \multirow{4}{\cellsmallwidth}{\textbf{Unseen \\Architec-\\ture}} & 
\multirow{4}{\celllargewidth}{SNGAN\cite{miyato2018spectral}, AttGAN\cite{he2019attgan}, \\ MMDGAN\cite{binkowski2018MMD},\\InfoMaxGAN\cite{lee2021infomax}} &
\multirow{4}{\celllargewidth}{StyleGAN2\cite{karras2020stylegan2}, \\ProGAN,\\ StyleGAN\cite{karras2019style}} &
\multirow{4}{\cellbigwidth}{S3GAN\cite{luvcic2019high},\\ BigGAN\cite{brock2018large},\\
ContraGAN\cite{kang2020contragan}} &
\multirow{4}{\cellbigwidth}{Wav2Lip\cite{prajwal2020lip}, \\FaceShifter\cite{li2019faceshifter}} &
\multirow{4}{\cellmidwidth}{SNGAN,\\InfoMaxGAN} & 
\multirow{4}{\cellmidwidth}{SNGAN, ProGAN,\\ MMDGAN,\\ StyleGAN2} & 
\multirow{4}{\cellmidwidth}{SNGAN, MMDGAN,\\ StyleGAN2,\\ StyleGAN3} \\\\\\\\
% % unseen dataset
\cmidrule{2-9}
& \multirow{2}{\cellsmallwidth}{\textbf{Unseen\\Dataset}} & 
\multicolumn{7}{c}{\multirow{2}{*}{ProGAN, StyleGAN, StyleGAN3 (Cow, Sheep, Classroom, Bridge, Kitchen, Airplane, Church)}} \\\\
% unseen real
\midrule
\multicolumn{2}{c}{\textbf{Unseen Real}} & 
\multicolumn{7}{c}{Coco, Summer}  \\
\bottomrule[1.5pt]
\end{tabular}}
\label{tab:dataset_1split}
\vspace{-5mm}
\end{table*}




==> Tables/dataset_3setup.tex <==

\begin{table*}
\small
\caption{List of dataset used in our experiments, including 4 groups: seen real, seen models, unseen real and unseen models.}
\begin{center}
\setlength\tabcolsep{1.0pt}
\begin{tabular}{llcc}
\toprule
\multirow{3}{2cm}{\textit{\textbf{Setup I: \\Cross-seed}}} & Dataset &  Seen Models  & Unseen Models \\
\cmidrule{2-4} 
& CelebA & ProGAN\_seed0, ProGAN\_seed1 &  ProGAN\_seed2 - ProGAN\_seed9 \\
& LSUN-bedroom & ProGAN\_seed0, ProGAN\_seed1 &  ProGAN\_seed2 - ProGAN\_seed9 \\
\midrule
\multirow{3}{2cm}{\textit{\textbf{Setup II: Cross-architecture}}} & Dataset &  Seen Models  & Unseen Models\\
\cmidrule{2-4} 
& CelebA & ProGAN, MMDGAN &  StarGAN, AttGAN, SNGAN, InfoMaxGAN \\
& Faces-HQ & StyleGAN2, StyleGAN3\_r & ProGAN, StyleGAN, StyleGAN3\_t \\
& ImageNet & SAGAN, BigGAN & S3GAN, SNGAN, ContraGAN \\
& LSUN-bedroom & SNGAN, ProGAN &  MMDGAN, InfoMaxGAN \\
& Youtube & Faceshifter, FaceSwap & FSGAN, Wav2Lip \\
\midrule
\multirow{3}{2cm}{\textit{\textbf{Setup III: Cross-dataset}}} & Architectures &  Training Datasets for Seen Models  & Training Datasets for Unseen Models\\
\cmidrule{2-4} 
& StyleGAN & Bus, Cat & Airplane, Bridge, Church Outdoor, Classroom, Cow, Kitchen, Sheep \\
& StyleGAN2 & Bus, Cat & Airplane, Bridge, Church Outdoor, Classroom, Cow, Kitchen, Sheep \\
& StyleGAN3 & Bus, Cat & Airplane, Bridge, Church Outdoor, Classroom, Cow, Kitchen, Sheep \\
\bottomrule
\end{tabular}
\end{center}
\label{tab:dataset_3setup}
\end{table*}


==> Tables/dataset_explain.tex <==
\begin{table}[t]
\setlength\tabcolsep{1.8pt}
\setlength{\abovecaptionskip}{2mm}
\caption{The relationship between Unseen Fake and Seen Fake.}
\centering
\scalebox{0.9}{
\begin{tabular}{l|ccc}
\toprule
 \multirow{3}{*}{\textbf{Unseen Fake}} & \multicolumn{3}{c}{\textbf{Relationship with Seen Fake}} \\
\cmidrule{2-4}
 & Seed & Architecture & Dataset \\
\midrule
\textbf{Unseen Seed} & Different & Same & Same \\
\textbf{Unseen Architecture} & - & Different & Same \\
\textbf{Unseen Dataset} & - & Same & Different \\
\bottomrule
\end{tabular}}
\label{tab:dataset_explain}
\vspace{-5mm}
\end{table}



==> Tables/dataset_explain_combine.tex <==



\begin{table}[t]
\setlength\tabcolsep{1.8pt}
\begin{center}
\scalebox{0.9}{
\begin{tabular}{l|ccc}
\toprule
 \multirow{2}{*}{\textbf{Unseen Fake}} & \multicolumn{3}{c}{\textbf{Relationship with Seen Fake}} \\
\cmidrule{2-4}
 & Seed & Architecture & Dataset \\
\midrule
\textbf{Unseen Seed} & Different & Same & Same \\
\textbf{Unseen Architecture} & - & Different & Same \\
\textbf{Unseen Dataset} & - & Same & Different \\
\bottomrule
\end{tabular}}
\end{center}
\caption{The relationship between seen fake and unseen fake.}
\label{tab:dataset_explain}
\end{table}


\begin{table}[t]
\setlength\tabcolsep{1.8pt}
\begin{center}
\begin{tabular}{ll|cc}
\toprule
\textbf{Split} & \textbf{Scenario} & \textbf{Data Type} \\
\midrule
\textbf{Train} & \textbf{Closed set} & Seen Real, Seen Fake \\
\cmidrule{1-2}
\multirow{2}{*}{\textbf{Test}} & \textbf{Closed set} & Seen Real, \textcolor{blue}{Unseen Real}, Seen Fake \\
\cmidrule{2-2}
& \textbf{Open set} & \textcolor{blue}{Unseen Fake} \\
%  \multirow{2}{*}{\textbf{Unseen Fake}} & \multicolumn{3}{c}{\textbf{Relationship with Seen Fake}} \\
% \cmidrule{2-4}
%  & Seed & Architecture & Dataset \\
% \midrule
% \textbf{Unseen Seed} & Different & Same & Same \\
% \textbf{Unseen Architecture} & - & Different & Same \\
% \textbf{Unseen Dataset} & - & Same & Different \\
\bottomrule
\end{tabular}
\end{center}
\caption{Data Split. The testing set includes closed-set and open-set scenarios.}
\label{tab:train_test_split}
\end{table}


==> Tables/dataset_split1.tex <==
\begin{table*}[t]
\setlength\tabcolsep{1.8pt}
\setlength{\abovecaptionskip}{2mm}
\caption{Split 1 of the OSMA benchmark.}
\centering
\scalebox{0.83}{
\begin{tabular}{lllllllll}
\toprule[1.5pt]
% seen real
\multicolumn{2}{c}{\textbf{Seen Real}} & CelebA & Face-HQ & ImageNet & Youtube & LSUN-Bedroom & LSUN-Cat & LSUN-Bus \\
% seen fake
\midrule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Seen Fake}}} &
\multirow{2}{\celllargewidth}{StarGAN\cite{choi2018stargan},\\ProGAN\_seed0\cite{karras2017progressive}} & \multirow{2}{\celllargewidth}{StyleGAN3-r\cite{karras2021alias}, \\StyleGAN3-t} & \multirow{2}{\cellbigwidth}{SAGAN\cite{zhang2019self},\\SNGAN} & 
\multirow{2}{\cellbigwidth}{FSGAN\cite{nirkin2019fsgan}, \\FaceSwap\cite{faceswap}} & 
\multirow{2}{\cellmidwidth}{ProGAN\_seed0, \\MMDGAN} & 
\multirow{2}{\cellmidwidth}{StyleGAN, \\StyleGAN3} & 
\multirow{2}{\cellmidwidth}{ProGAN, \\StyleGAN} \\ \\
% unseen fake
% % unseen seed
\midrule
\multirow{8}{\cellsmallwidth}{\textbf{Unseen \\Fake}} & \multirow{2}{\cellsmallwidth}{\textbf{Unseen \\Seed}} &
\multirow{2}{\celllargewidth}{ProGAN\\(seed1,2,3,4,5)} & 
\multirow{2}{\celllargewidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{ProGAN\\(seed1,2,3,4,5)} & 
\multirow{2}{\cellmidwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{\centering -} \\\\
% % unseen arch
\cmidrule{2-9}
& \multirow{4}{\cellsmallwidth}{\textbf{Unseen \\Architec-\\ture}} & 
\multirow{4}{\celllargewidth}{SNGAN\cite{miyato2018spectral}, AttGAN\cite{he2019attgan}, \\ MMDGAN\cite{binkowski2018MMD},\\InfoMaxGAN\cite{lee2021infomax}} &
\multirow{4}{\celllargewidth}{StyleGAN2\cite{karras2020stylegan2}, \\ProGAN,\\ StyleGAN\cite{karras2019style}} &
\multirow{4}{\cellbigwidth}{S3GAN\cite{luvcic2019high},\\ BigGAN\cite{brock2018large},\\
ContraGAN\cite{kang2020contragan}} &
\multirow{4}{\cellbigwidth}{Wav2Lip\cite{prajwal2020lip}, \\FaceShifter\cite{li2019faceshifter}} &
\multirow{4}{\cellmidwidth}{SNGAN,\\InfoMaxGAN} & 
\multirow{4}{\cellmidwidth}{SNGAN, ProGAN,\\ MMDGAN,\\ StyleGAN2} & 
\multirow{4}{\cellmidwidth}{SNGAN, MMDGAN,\\ StyleGAN2,\\ StyleGAN3} \\\\\\\\
% % unseen dataset
\cmidrule{2-9}
& \multirow{2}{\cellsmallwidth}{\textbf{Unseen\\Dataset}} & 
\multicolumn{7}{c}{\multirow{2}{*}{ProGAN, StyleGAN, StyleGAN3 (Cow, Sheep, Classroom, Bridge, Kitchen, Airplane, Church)}} \\\\
% unseen real
\midrule
\multicolumn{2}{c}{\textbf{Unseen Real}} & 
\multicolumn{7}{c}{Coco, Summer}  \\
\bottomrule[1.5pt]
\end{tabular}}
\label{tab:dataset_split1}
% \vspace{-5mm}
\end{table*}




==> Tables/dataset_split1_bak.tex <==
% \begin{table*}
% % \small
% \caption{List of dataset used in our experiments, including 4 groups: seen real, seen models, unseen real and unseen models.} 
% \setlength\tabcolsep{2pt}
% \begin{center}
% % \begin{tabular}{p{2.5cm}<{\centering}p{4cm}<{\centering}p{4cm}<{\centering}p{3.6cm}<{\centering}p{4cm}<{\centering}p{3cm}<{\centering}}
% \scalebox{0.9}{
% \begin{tabular}{p{1.5cm}p{4cm}p{4cm}p{3.8cm}p{3cm}p{2cm}}
% \toprule[1.5pt]
% \multirow{2}{1.5cm}{\textbf{Seen Real}} & \multirow{2}{4cm}{\textbf{Seen Models}} & \multicolumn{3}{c}{\textbf{Unseen Models}} & \multirow{2}{2cm}{\textbf{Unseen Real}} \\
% \cmidrule{3-5} 
%  & & \textbf{Unseen Seed} & \textbf{Unseen Architecture} & \textbf{Unseen Dataset} & \\
% \midrule[1pt]
% \multirow{2}{2cm}{CelebA} & \multirow{2}{4cm}{ProGAN (s0), StarGAN} &  \multirow{2}{4cm}{ProGAN (s1, s2, s3, s4, s5)} & \multirow{2}{3.8cm}{SNGAN, AttGAN, MMDGAN, InfoMaxGAN} & \multirow{15}{3cm}{ProGAN, StyleGAN, StyleGAN3 (Cow, Sheep, Classroom, Bridge, Kitchen, Airplane, Church)}
% & \multirow{15}{2cm}{VGG, GTA, CoCo}\\ \\
% \cdashline{1-4}
% \multirow{2}{2cm}{Faces-HQ} & \multirow{2}{4cm}{StyleGAN3-r, StyleGAN3-t} &  \multirow{2}{4cm}{\centering -} & \multirow{2}{3.5cm}{StyleGAN2, ProGAN, StyleGAN} &  \\ \\
% \cdashline{1-4}
% \multirow{2}{2cm}{ImageNet} & \multirow{2}{4cm}{SNGAN, SAGAN} &  \multirow{2}{4cm}{\centering -} & \multirow{2}{3.5cm}{S3GAN, BigGAN, ContraGAN} &  \\ \\
% \cdashline{1-4}
% \multirow{2}{2cm}{Youtube} & \multirow{2}{4cm}{FSGAN, FaceSwap} & \multirow{2}{4cm}{\centering -} & \multirow{2}{3.5cm}{Wav2Lip, Faceshifter} \\ \\
% \cdashline{1-4}
% \multirow{2}{2cm}{LSUN Bedroom} & \multirow{2}{4cm}{ProGAN (s0), MMDGAN} &  \multirow{2}{4cm}{ProGAN (s1, s2, s3, s4, s5)} & \multirow{2}{3.5cm}{SNGAN, InfoMaxGAN} & \\ \\
% \cdashline{1-4}
% \multirow{2}{2cm}{LSUN \\Cat} & \multirow{2}{4cm}{StyleGAN, StyleGAN3} &  \multirow{2}{4cm}{\centering -} & \multirow{2}{3.5cm}{SNGAN, ProGAN, MMDGAN, StyleGAN2} & \\ \\
% \cdashline{1-4}
% \multirow{2}{2cm}{LSUN \\Bus} & \multirow{2}{4cm}{ProGAN, StyleGAN} &  \multirow{2}{4cm}{\centering -} & \multirow{2}{3.8cm}{SNGAN, MMDGAN, StyleGAN2, StyleGAN3} & \\ \\
% \bottomrule[1.5pt]
% \end{tabular}}
% \end{center}
% \label{tab:dataset_split1}
% \end{table*}

\begin{table*}
% \small
\caption{One split of of open-set model attribution benchmark, including 4 groups: seen real, seen fake, unseen real and unseen fake.} 
\setlength\tabcolsep{2pt}
\begin{center}
% \begin{tabular}{p{2.5cm}<{\centering}p{4cm}<{\centering}p{4cm}<{\centering}p{3.6cm}<{\centering}p{4cm}<{\centering}p{3cm}<{\centering}}
\scalebox{0.9}{
\begin{tabular}{p{1.8cm}p{3cm}p{4cm}p{4.8cm}p{3cm}p{2cm}}

\toprule[1.5pt]
\multirow{2}{1.5cm}{\textbf{Seen Real}} & \multirow{2}{4cm}{\textbf{Seen Fake}} & \multicolumn{3}{c}{\textbf{Unseen Fake}} & \multirow{2}{2cm}{\textbf{Unseen Real}} \\
\cmidrule{3-5} 
 & & \textbf{Unseen Seed} & \textbf{Unseen Architecture} & \textbf{Unseen Dataset} & \\
\midrule[1pt]
\multirow{2}{2cm}{CelebA} & \multirow{2}{4cm}{StarGAN\cite{choi2018stargan},\\ProGAN\cite{karras2017progressive} (s0)} &  \multirow{2}{4cm}{ProGAN (s1, s2, s3, s4, s5)} & \multirow{2}{5cm}{SNGAN\cite{miyato2018spectral}, MMDGAN\cite{binkowski2018MMD}, AttGAN\cite{he2019attgan}, InfoMaxGAN\cite{lee2021infomax}} & \multirow{15}{3cm}{ProGAN, StyleGAN, StyleGAN3 (Cow, Sheep, Classroom, Bridge, Kitchen, Airplane, Church)}
& \multirow{15}{2cm}{CoCo, Summer}\\ \\
\cdashline{1-4}
\multirow{2}{2cm}{Face-HQ} & \multirow{2}{4cm}{StyleGAN3-r\cite{karras2021alias}, \\StyleGAN3-t} &  \multirow{2}{4cm}{\centering -} & \multirow{2}{5cm}{StyleGAN2\cite{karras2020stylegan2}, \\ProGAN, StyleGAN\cite{karras2019style}} &  \\ \\
\cdashline{1-4}
\multirow{2}{2cm}{ImageNet} & \multirow{2}{4cm}{SAGAN\cite{zhang2019self},\\SNGAN} &  \multirow{2}{4cm}{\centering -} & \multirow{2}{5cm}{S3GAN\cite{luvcic2019high},\\ BigGAN\cite{brock2018large}, ContraGAN\cite{kang2020contragan}} &  \\ \\
\cdashline{1-4}
\multirow{2}{2cm}{Youtube} & \multirow{2}{4cm}{FSGAN\cite{nirkin2019fsgan}, \\FaceSwap\cite{faceswap}} & \multirow{2}{4cm}{\centering -} & \multirow{2}{5cm}{Wav2Lip\cite{prajwal2020lip}, \\FaceShifter\cite{li2019faceshifter}} \\ \\
\cdashline{1-4}
\multirow{2}{2cm}{LSUN Bedroom} & \multirow{2}{4cm}{ProGAN (s0), \\MMDGAN} &  \multirow{2}{4cm}{ProGAN (s1, s2, s3, s4, s5)} & \multirow{2}{4cm}{SNGAN, \\InfoMaxGAN} & \\ \\
\cdashline{1-4}
\multirow{2}{2cm}{LSUN \\Cat} & \multirow{2}{4cm}{StyleGAN, \\StyleGAN3} &  \multirow{2}{4cm}{\centering -} & \multirow{2}{5cm}{SNGAN, ProGAN, \\MMDGAN, StyleGAN2} & \\ \\
\cdashline{1-4}
\multirow{2}{2cm}{LSUN \\Bus} & \multirow{2}{4cm}{ProGAN, \\StyleGAN} &  \multirow{2}{4cm}{\centering -} & \multirow{2}{5cm}{SNGAN, MMDGAN, \\StyleGAN2, StyleGAN3} & \\ \\
\bottomrule[1.5pt]
\end{tabular}}
\end{center}
\label{tab:dataset_split1_bak}
\end{table*}


\begin{table*}
% \small
\caption{One split of of open-set model attribution benchmark, including 4 groups: seen real, seen fake, unseen real and unseen fake.} 
\setlength\tabcolsep{2pt}
\begin{center}
% \begin{tabular}{p{2.5cm}<{\centering}p{4cm}<{\centering}p{4cm}<{\centering}p{3.6cm}<{\centering}p{4cm}<{\centering}p{3cm}<{\centering}}
\scalebox{0.9}{
\begin{tabular}{p{4cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
\toprule[1.5pt]
\textbf{Seen Real} & CelebA & Face-HQ & ImageNet & Youtube & LSUNBedroom & LSUN Cat & LSUN Bus\\
\multirow{2}{*}{\textbf{Seen Fake}} & \multirow{2}{*}{StarGAN\cite{choi2018stargan},\\ProGAN\cite{karras2017progressive} (s0)} & \multirow{2}{*}{StyleGAN3-r\cite{karras2021alias}, \\StyleGAN3-t} & \multirow{2}{*}{SAGAN\cite{zhang2019self},\\SNGAN} & \multirow{2}{*}{FSGAN\cite{nirkin2019fsgan}, \\FaceSwap\cite{faceswap}} & \multirow{2}{*}{ProGAN (s0), \\MMDGAN} & \multirow{2}{*}{StyleGAN, \\StyleGAN3} & \multirow{2}{*}{ProGAN, \\StyleGAN} \\
\multicolumn{2}{\multirow{7}{*}{\textbf{Unseen \\Fake}} & \multirow{2}{*}{\textbf{Unseen \\Seed}}} & \multirow{2}{*}{ProGAN\\(s1,s2,s3,s4,s5)} & \multirow{2}{*}{\centering -} & \multirow{2}{*}{\centering -} & \multirow{2}{*}{\centering -} & \multirow{2}{*}{ProGAN\\(s1,s2,s3,s4,s5)} & \multirow{2}{*}{\centering -} & \multirow{2}{*}{\centering -} \\
\multicolumn{2}{ &\multirow{3}{*}{\textbf{Unseen \\Architec\\-ture}}} & \multirow{3}{*}{SNGAN\cite{miyato2018spectral}, AttGAN\cite{he2019attgan}, \\ MMDGAN\cite{binkowski2018MMD},\\InfoMaxGAN\cite{lee2021infomax}} & \multirow{3}{*}{StyleGAN2\cite{karras2020stylegan2}, \\ProGAN,\\ StyleGAN\cite{karras2019style}} & \multirow{3}{*}{S3GAN\cite{luvcic2019high},\\ BigGAN\cite{brock2018large},\\ ContraGAN\cite{kang2020contragan}} &\multirow{3}{*}{Wav2Lip\cite{prajwal2020lip}, \\FaceShifter\cite{li2019faceshifter}} & \multirow{3}{*}{SNGAN,\\InfoMaxGAN} & \multirow{3}{*}{SNGAN, ProGAN,\\ MMDGAN,\\ StyleGAN2} & \multirow{3}{*}{SNGAN, MMDGAN,\\ StyleGAN2,\\ StyleGAN3} \\
\multicolumn{2}{&\multirow{2}{*}{\textbf{Unseen\\Dataset}}} & \multirow{2}{*}{ProGAN, StyleGAN, StyleGAN3(Cow, Sheep, Classroom, Bridge, Kitchen, Airplane, Church)} \\
\textbf{Unseen Real} & Coco, Summer \\

\bottomrule[1.5pt]
\end{tabular}}
\end{center}
\label{tab:dataset_split1_bak}
\end{table*}

==> Tables/dataset_split2.tex <==
\begin{table*}[t]
\setlength\tabcolsep{1.8pt}
\setlength{\abovecaptionskip}{2mm}
\caption{Split 2 of the OSMA benchmark}
\centering
\scalebox{0.83}{
\begin{tabular}{lllllllll}
\toprule[1.5pt]
% seen real
\multicolumn{2}{c}{\textbf{Seen Real}} & CelebA & Face-HQ & ImageNet & Youtube & LSUN-Bedroom & LSUN-Cat & LSUN-Bus \\
% seen fake
\midrule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Seen Fake}}} &
\multirow{2}{\celllargewidth}{InfoMaxGAN\cite{lee2021infomax},\\ProGAN\_seed1\cite{karras2017progressive}} & \multirow{2}{\celllargewidth}{StyleGAN\cite{karras2019style}, \\StyleGAN3-t\cite{karras2021alias}} & \multirow{2}{\cellbigwidth}{ContraGAN\cite{kang2020contragan},\\SNGAN} & 
\multirow{2}{\cellbigwidth}{FSGAN\cite{nirkin2019fsgan}, \\FaceShifter\cite{li2019faceshifter}} & 
\multirow{2}{\cellmidwidth}{SNGAN, \\ProGAN\_seed1} & 
\multirow{2}{\cellmidwidth}{SNGAN, \\StyleGAN2} & 
\multirow{2}{\cellmidwidth}{StyleGAN, \\StyleGAN3} \\ \\
% unseen fake
% % unseen seed
\midrule
\multirow{8}{\cellsmallwidth}{\textbf{Unseen \\Fake}} & \multirow{2}{\cellsmallwidth}{\textbf{Unseen \\Seed}} &
\multirow{2}{\celllargewidth}{ProGAN\\(seed0,2,3,4,5)} & 
\multirow{2}{\celllargewidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{ProGAN\\(seed0,2,3,4,5)} & 
\multirow{2}{\cellmidwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{\centering -} \\\\
% % unseen arch
\cmidrule{2-9}
& \multirow{4}{\cellsmallwidth}{\textbf{Unseen \\Architec-\\ture}} & 
\multirow{4}{\celllargewidth}{SNGAN\cite{miyato2018spectral}, AttGAN\cite{he2019attgan}, \\ MMDGAN\cite{binkowski2018MMD},\\StarGAN\cite{choi2018stargan}} &
\multirow{4}{\celllargewidth}{ProGAN, \\StyleGAN2\cite{karras2020stylegan2}, \\ StyleGAN3-r} &
\multirow{4}{\cellbigwidth}{S3GAN\cite{luvcic2019high},\\ BigGAN\cite{brock2018large},\\
SAGAN\cite{zhang2019self}} &
\multirow{4}{\cellbigwidth}{Wav2Lip\cite{prajwal2020lip}, \\FaceSwap\cite{faceswap}} &
\multirow{4}{\cellmidwidth}{MMDGAN,\\InfoMaxGAN} & 
\multirow{4}{\cellmidwidth}{ProGAN,\\ MMDGAN,\\ StyleGAN,\\ StyleGAN3} & 
\multirow{4}{\cellmidwidth}{ProGAN, \\ SNGAN,\\ MMDGAN,\\ StyleGAN2} \\\\\\\\
% % unseen dataset
\cmidrule{2-9}
& \multirow{2}{\cellsmallwidth}{\textbf{Unseen\\Dataset}} & 
\multicolumn{7}{c}{\multirow{2}{*}{SNGAN, StyleGAN, StyleGAN3 (Cow, Sheep, Classroom, Bridge, Kitchen, Airplane, Church)}} \\\\
% unseen real
\midrule
\multicolumn{2}{c}{\textbf{Unseen Real}} & 
\multicolumn{7}{c}{Coco, Summer}  \\
\bottomrule[1.5pt]
\end{tabular}}
\label{tab:dataset_split2}
% \vspace{-5mm}
\end{table*}




==> Tables/dataset_split3.tex <==
\begin{table*}[t]
\setlength\tabcolsep{1.8pt}
\setlength{\abovecaptionskip}{2mm}
\caption{Split 3 of the OSMA benchmark}
\centering
\scalebox{0.83}{
\begin{tabular}{lllllllll}
\toprule[1.5pt]
% seen real
\multicolumn{2}{c}{\textbf{Seen Real}} & CelebA & Face-HQ & ImageNet & Youtube & LSUN-Bedroom & LSUN-Cat & LSUN-Bus \\
% seen fake
\midrule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Seen Fake}}} &
\multirow{2}{\celllargewidth}{AttGAN\cite{he2019attgan}, \\ProGAN\_seed2\cite{karras2017progressive}} & \multirow{2}{\celllargewidth}{ProGAN, \\StyleGAN3-t\cite{karras2021alias}} & \multirow{2}{\cellbigwidth}{S3GAN\cite{luvcic2019high},\\SNGAN} & 
\multirow{2}{\cellbigwidth}{FaceSwap\cite{faceswap}, \\FaceShifter\cite{li2019faceshifter}} & 
\multirow{2}{\cellmidwidth}{InfoMaxGAN, \\ProGAN\_seed2} & 
\multirow{2}{\cellmidwidth}{SNGAN, ProGAN\\} & 
\multirow{2}{\cellmidwidth}{ProGAN, \\MMDGAN} \\ \\
% unseen fake
% % unseen seed
\midrule
\multirow{8}{\cellsmallwidth}{\textbf{Unseen \\Fake}} & \multirow{2}{\cellsmallwidth}{\textbf{Unseen \\Seed}} &
\multirow{2}{\celllargewidth}{ProGAN\\(seed0,1,3,4,5)} & 
\multirow{2}{\celllargewidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{ProGAN\\(seed0,1,3,4,5)} & 
\multirow{2}{\cellmidwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{\centering -} \\\\
% % unseen arch
\cmidrule{2-9}
& \multirow{4}{\cellsmallwidth}{\textbf{Unseen \\Architec-\\ture}} & 
\multirow{4}{\celllargewidth}{SNGAN\cite{miyato2018spectral}, InfoMaxGAN\cite{lee2021infomax},\\ MMDGAN\cite{binkowski2018MMD},\\StarGAN\cite{choi2018stargan}} &
\multirow{4}{\celllargewidth}{StyleGAN\cite{karras2019style}, \\StyleGAN2\cite{karras2020stylegan2}, \\ StyleGAN3-r} &
\multirow{4}{\cellbigwidth}{ContraGAN\cite{kang2020contragan},\\ BigGAN\cite{brock2018large},\\ SAGAN\cite{zhang2019self}} &
\multirow{4}{\cellbigwidth}{Wav2Lip\cite{prajwal2020lip}, FSGAN\cite{nirkin2019fsgan}} &
\multirow{4}{\cellmidwidth}{MMDGAN,\\SNGAN} & 
\multirow{4}{\cellmidwidth}{StyleGAN2,\\ MMDGAN,\\ StyleGAN,\\ StyleGAN3} & 
\multirow{4}{\cellmidwidth}{SNGAN,\\StyleGAN,\\StyleGAN3,\\StyleGAN2}\\\\\\\\
% % unseen dataset
\cmidrule{2-9}
& \multirow{2}{\cellsmallwidth}{\textbf{Unseen\\Dataset}} & 
\multicolumn{7}{c}{\multirow{2}{*}{SNGAN, MMDGAN, ProGAN (Cow, Sheep, Classroom, Bridge, Kitchen, Airplane, Church)}} \\\\
% unseen real
\midrule
\multicolumn{2}{c}{\textbf{Unseen Real}} & 
\multicolumn{7}{c}{Coco, Summer}  \\
\bottomrule[1.5pt]
\end{tabular}}
\label{tab:dataset_split3}
% \vspace{-5mm}
\end{table*}




==> Tables/dataset_split4.tex <==
\begin{table*}[t]
\setlength\tabcolsep{1.8pt}
\setlength{\abovecaptionskip}{2mm}
\caption{Split 4 of the OSMA benchmark}
\centering
\scalebox{0.83}{
\begin{tabular}{lllllllll}
\toprule[1.5pt]
% seen real
\multicolumn{2}{c}{\textbf{Seen Real}} & CelebA & Face-HQ & ImageNet & Youtube & LSUN-Bedroom & LSUN-Cat & LSUN-Bus \\
% seen fake
\midrule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Seen Fake}}} &
\multirow{2}{\celllargewidth}{SNGAN\cite{miyato2018spectral}, \\ProGAN\_seed3\cite{karras2017progressive}} & \multirow{2}{\celllargewidth}{ProGAN, \\StyleGAN3-r\cite{karras2021alias}} & \multirow{2}{\cellbigwidth}{ContraGAN\cite{kang2020contragan},\\ BigGAN\cite{brock2018large}} & 
\multirow{2}{\cellbigwidth}{Wav2Lip\cite{prajwal2020lip}, FSGAN\cite{nirkin2019fsgan}} & 
\multirow{2}{\cellmidwidth}{SNGAN, \\ProGAN\_seed3} & 
\multirow{2}{\cellmidwidth}{ProGAN, \\MMDGAN} & 
\multirow{2}{\cellmidwidth}{SNGAN, \\MMDGAN} \\ \\
% unseen fake
% % unseen seed
\midrule
\multirow{8}{\cellsmallwidth}{\textbf{Unseen \\Fake}} & \multirow{2}{\cellsmallwidth}{\textbf{Unseen \\Seed}} &
\multirow{2}{\celllargewidth}{ProGAN\\(seed0,1,2,4,5)} & 
\multirow{2}{\celllargewidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{ProGAN\\(seed0,1,2,4,5)} & 
\multirow{2}{\cellmidwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{\centering -} \\\\
% % unseen arch
\cmidrule{2-9}
& \multirow{4}{\cellsmallwidth}{\textbf{Unseen \\Architec-\\ture}} & 
\multirow{4}{\celllargewidth}{AttGAN\cite{he2019attgan}, InfoMaxGAN\cite{lee2021infomax},\\ MMDGAN\cite{binkowski2018MMD},\\StarGAN\cite{choi2018stargan}} &
\multirow{4}{\celllargewidth}{StyleGAN\cite{karras2019style}, \\StyleGAN2\cite{karras2020stylegan2}, \\ StyleGAN3-t} &
\multirow{4}{\cellbigwidth}{S3GAN\cite{luvcic2019high},\\SNGAN,\\ SAGAN\cite{zhang2019self}} &
\multirow{4}{\cellbigwidth}{FaceSwap\cite{faceswap}, \\FaceShifter\cite{li2019faceshifter}} &
\multirow{4}{\cellmidwidth}{MMDGAN,\\InfoMaxGAN} & 
\multirow{4}{\cellmidwidth}{SNGAN,\\StyleGAN, \\StyleGAN2,\\ StyleGAN3} & 
\multirow{4}{\cellmidwidth}{ProGAN,\\StyleGAN,\\StyleGAN2,\\StyleGAN3}\\\\\\\\
% % unseen dataset
\cmidrule{2-9}
& \multirow{2}{\cellsmallwidth}{\textbf{Unseen\\Dataset}} & 
\multicolumn{7}{c}{\multirow{2}{*}{SNGAN, ProGAN, MMDGAN (Cow, Sheep, Classroom, Bridge, Kitchen, Airplane, Church)}} \\\\
% unseen real
\midrule
\multicolumn{2}{c}{\textbf{Unseen Real}} & 
\multicolumn{7}{c}{Coco, Summer}  \\
\bottomrule[1.5pt]
\end{tabular}}
\label{tab:dataset_split4}
% \vspace{-5mm}
\end{table*}




==> Tables/dataset_split5.tex <==
\begin{table*}[t]
\setlength\tabcolsep{1.8pt}
\setlength{\abovecaptionskip}{2mm}
\caption{Split 5 of the OSMA benchmark}
\centering
\scalebox{0.83}{
\begin{tabular}{lllllllll}
\toprule[1.5pt]
% seen real
\multicolumn{2}{c}{\textbf{Seen Real}} & CelebA & Face-HQ & ImageNet & Youtube & LSUN-Bedroom & LSUN-Cat & LSUN-Bus \\
% seen fake
\midrule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Seen Fake}}} &
\multirow{2}{\celllargewidth}{AttGAN\cite{he2019attgan}, \\ProGAN\_seed4\cite{karras2017progressive}} & \multirow{2}{\celllargewidth}{StyleGAN\cite{karras2019style}, \\StyleGAN3-t\cite{karras2021alias}} & \multirow{2}{\cellbigwidth}{ContraGAN\cite{kang2020contragan},\\ BigGAN\cite{brock2018large}} & 
\multirow{2}{\cellbigwidth}{FaceSwap\cite{faceswap}, \\Wav2Lip\cite{prajwal2020lip}} & 
\multirow{2}{\cellmidwidth}{InfoMaxGAN, \\ProGAN\_seed4} & 
\multirow{2}{\cellmidwidth}{StyleGAN, ProGAN\\} & 
\multirow{2}{\cellmidwidth}{ProGAN, \\MMDGAN} \\ \\
% unseen fake
% % unseen seed
\midrule
\multirow{8}{\cellsmallwidth}{\textbf{Unseen \\Fake}} & \multirow{2}{\cellsmallwidth}{\textbf{Unseen \\Seed}} &
\multirow{2}{\celllargewidth}{ProGAN\\(seed0,1,2,3,5)} & 
\multirow{2}{\celllargewidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellbigwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{ProGAN\\(seed0,1,2,3,5)} & 
\multirow{2}{\cellmidwidth}{\centering -} & 
\multirow{2}{\cellmidwidth}{\centering -} \\\\
% % unseen arch
\cmidrule{2-9}
& \multirow{4}{\cellsmallwidth}{\textbf{Unseen \\Architec-\\ture}} & 
\multirow{4}{\celllargewidth}{SNGAN\cite{miyato2018spectral}, InfoMaxGAN\cite{lee2021infomax},\\ MMDGAN\cite{binkowski2018MMD},\\StarGAN\cite{choi2018stargan}} &
\multirow{4}{\celllargewidth}{ProGAN, \\StyleGAN2\cite{karras2020stylegan2}, \\ StyleGAN3-r} &
\multirow{4}{\cellbigwidth}{S3GAN\cite{luvcic2019high},\\SNGAN,\\ SAGAN\cite{zhang2019self}} &
\multirow{4}{\cellbigwidth}{FaceShifter\cite{li2019faceshifter}, FSGAN\cite{nirkin2019fsgan}} &
\multirow{4}{\cellmidwidth}{MMDGAN,\\SNGAN} & 
\multirow{4}{\cellmidwidth}{StyleGAN2,\\ MMDGAN,\\ SNGAN,\\ StyleGAN3} & 
\multirow{4}{\cellmidwidth}{SNGAN,\\StyleGAN,\\StyleGAN3,\\StyleGAN2}\\\\\\\\
% % unseen dataset
\cmidrule{2-9}
& \multirow{2}{\cellsmallwidth}{\textbf{Unseen\\Dataset}} & 
\multicolumn{7}{c}{\multirow{2}{*}{ProGAN, MMDGAN, StyleGAN (Cow, Sheep, Classroom, Bridge, Kitchen, Airplane, Church)}} \\\\
% unseen real
\midrule
\multicolumn{2}{c}{\textbf{Unseen Real}} & 
\multicolumn{7}{c}{Coco, Summer}  \\
\bottomrule[1.5pt]
\end{tabular}}
\label{tab:dataset_split5}
% \vspace{-5mm}
\end{table*}




==> Tables/train_test_split.tex <==


\begin{table}[t]
\setlength\tabcolsep{1.8pt}
\setlength{\abovecaptionskip}{2mm}
\caption{Data split for training and testing process.}
\centering
\scalebox{0.9}{
\begin{tabular}{ll|cc}
\toprule
 & \textbf{} & \textbf{Data Group} \\
\midrule 
\textbf{Train} & \textbf{Closed-Set} & Seen Real, Seen Fake \\
\midrule 
\multirow{2}{*}{\textbf{Test}} & \textbf{Closed-Set} & Seen Real, \textcolor{KnownColor}{Unseen Real}, Seen Fake \\
& \textbf{Open-Set} & \textcolor{KnownColor}{Unseen Fake} \\
\bottomrule
\end{tabular}}
\label{tab:train_test_split}
\vspace{-5mm}
\end{table}



==> macros.tex <==
\usepackage{ifthen}
\usepackage{xcolor}

\definecolor{YunColor}{rgb}{0.0,0.1,0.9}
\definecolor{FanColor}{rgb}{0.8,0,0.8}
\definecolor{WDDColor}{rgb}{0,0.8,0.8}
\definecolor{YTYColor}{rgb}{0.8,0,0}
\definecolor{KnownColor}{rgb}{0.12,0.47,0.7}

\newcommand{\increase}[1]{{\color{teal}(+#1)}}
\newcommand{\decrease}[1]{{\color{red}(-#1)}}

\newcommand{\yun}[1]{{\color{YunColor}[Yun: #1]}}

\newcommand{\fan}[1]{{\color{FanColor}[Fan: #1]}}
\newcommand{\wdd}[1]{{\color{WDDColor}[WDD: #1]}}
\newcommand{\yty}[1]{{\color{YTYColor}[yty: #1]}}

\newcommand{\revision}[1]{{\color{blue}#1}}

\newcommand{\warning}[1]{{\it\color{red} #1}}
\newcommand{\toremove}[1]{{\it\color{red} (To remove) #1}}
\newcommand{\note}[1]{{\it\color{blue} #1}}
\newcommand{\nothing}[1]{}

\newcommand\celllargewidth{2.9cm}
\newcommand\cellbigwidth{2.4cm}
\newcommand\cellmidwidth{2cm}
\newcommand\cellsmallwidth{1.5cm}


\ifthenelse{\equal{\final}{1}}
{

\renewcommand{\fan}[1]{}
\renewcommand{\yun}[1]{}
\renewcommand{\wdd}[1]{}

\renewcommand{\warning}[1]{}
\renewcommand{\toremove}[1]{}
\renewcommand{\note}[1]{}
\renewcommand{\nothing}[1]{}
\renewcommand{\revision}[1]{#1}
}{}

\hyphenpenalty=1000 % magic number to reduce ugly line breaks

\newcommand{\inputsection}[1]{\input{Sections/#1}}
\newcommand{\inputfigure}[1]{\input{Figures/#1}}
\newcommand{\inputtable}[1]{\input{Tables/#1}}


\newcommand{\figtext}[1]{{\footnotesize #1}}
\newcommand{\smallfigtext}[1]{{\scriptsize #1}}

\newcommand{\etal}[0]{~et al.}
\newcommand{\wrt}[0]{~w.r.t.}
\newcommand{\ie}[0]{~i.e.}
\newcommand{\eg}[0]{~e.g.}


 

